Total-Decom: Decomposed 3D Scene Reconstruction with Minimal Interaction

Scene reconstruction from multi-view images is a fundamental problem in computer vision and graphics. Recent neural implicit surface reconstruction methods have achieved high-quality results; however, editing and manipulating the 3D geometry of reconstructed scenes remains challenging due to the absence of naturally decomposed object entities and complex object/background compositions. In this paper, we present Total-Decom, a novel method for decomposed 3D reconstruction with minimal human interaction. Our approach seamlessly integrates the Segment Anything Model (SAM) with hybrid implicit-explicit neural surface representations and a mesh-based region-growing technique for accurate 3D object decomposition. Total-Decom requires minimal human annotations while providing users with real-time control over the granularity and quality of decomposition. We extensively evaluate our method on benchmark datasets and demonstrate its potential for downstream applications, such as animation and scene editing. The code is available at https://github.com/CVMI-Lab/Total-Decom.git.

==> sec/0_abstract.tex <==
\begin{abstract}
Scene reconstruction from multi-view images is a fundamental problem in computer vision and graphics. Recent neural implicit surface reconstruction methods have achieved high-quality results; however, editing and manipulating the 3D geometry of reconstructed scenes remains challenging due to the absence of naturally decomposed object entities and complex object/background compositions. 
% Briefly introduce the research question/focus to make the task clear
%
%Neural implicit surface is a fascinating method to represent a scene, enabling high fidelity reconstruction.
%However, decomposing the extracted surface is challenging as the entire scene are represented by a holistic mesh which are not compositional.
% Point out the weakness of previous work
% Main weakness 1: Uncontrolled Scalability
%
%Existing methods utilize separate neural networks to represent individual objects, leading to scalability issues, as the network size must increase with the number of object instances. 
% Main weakness 2: acquisition of labels
%
%Additionally, they rely on multi-view consistent instance-level dense labels, which are difficult to acquire in real-world scenes. %, further limiting their downstream applications.
% Motivation and a brief introduction to our solution
%
In this paper, we present Total-Decom, a novel method for decomposed 3D reconstruction with minimal human interaction.
%To address these challenges, this paper introduces a novel method that can reconstruct the holistic scene and decompose it in a complete manner. %, while ensuring the plausibility of the occluded surfaces in the background of the scene.
% Overview of the pipeline
%
Our approach seamlessly integrates the Segment Anything Model (SAM) with hybrid implicit-explicit neural surface representations and a mesh-based region-growing technique for accurate 3D object decomposition.  
Total-Decom requires minimal human annotations while providing users with real-time control over the granularity and quality of decomposition. We extensively evaluate our method on benchmark datasets and demonstrate its potential for downstream applications, such as animation and scene editing. Codes will be made publicly available. 

 %while requiring minimal human annotations. 
%We first represent the entire scene in a bilayer form, leveraging depth and semantic information to ensure that objects in the scene can be distinguished from the background, e.g., walls or floors, which belong to a different layer. %, and optimize the surfaces belonging to each layer separately. 
%Scenic priors, particularly plane constraints, are employed to facilitate high-quality reconstruction in occluded regions.
%We further integrate 2D general features from the segment anything model, allowing users to interactively select any object in the scene.
%Our method further propagates the 2D user-specified 'objectness' through neural implicit representation to the 3D space, using a novel neural surface region growing algorithm to extract the corresponding 3D object without additional interaction. 
% Illustrate the result and address the two weakness once again
%
%Extensive experimental results validate the effectiveness of our approach, showcasing its ability to generate high-fidelity outputs for complex holistic scenes and handle a large number of objects without need of instance-level labels.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Scene reconstruction from multi-view images is a fundamental problem in computer vision and graphics~\cite{schoenberger2016sfm, schoenberger2016mvs, Local_Implicit_Grid_CVPR20, peng2020convolutional, huang2023nksr, oechsle2021unisurf}. 
Recently, neural implicit surface reconstruction methods such as VolSDF~\cite{yariv2021volume} and NeuS~\cite{wang2021neus} have been proposed to address this problem and have achieved high-quality results. 
However, editing and manipulating the 3D geometry of a reconstructed scene remains challenging due to the absence of naturally decomposed object entities and complex object/background compositions. 
Such functionality is, however, desired for many real-world applications, such as editing, animation, and simulation. 
Consequently, we are motivated to investigate decomposed 3D reconstruction, which enables the extraction of desired object-level shapes and facilitates scene manipulations such as reorganizing objects in a scene (see Fig.~\ref{fig:teaser}).
\begin{comment}
Scene reconstruction from sparse multi-view images has been a fundamental problem in computer vision and graphics~\cite{schoenberger2016sfm, schoenberger2016mvs, Local_Implicit_Grid_CVPR20}.
Recently, neural implicit surface representations such as VolSDF~\cite{yariv2021volume}, NeuS~\cite{wang2021neus}, UNISURF~\cite{oechsle2021unisurf} have been proposed for this task.
Despite advancements, editing/manipulating the 3D geometry of a reconstructed scene, a desired function for real-world applications such as animation and embodied simulation, remains a challenging problem as it doesn't naturally offer decomposed objects.  
This motivates us to study decomposed 3D reconstruction, which allows us to obtain the shape of desired objects and perform manipulations such as object movement (see Figure xxx).  
\end{comment}
%, an under-explored yet important problem for many real-world applications such as animation and embodied simulation.
%{Although advancements has been achieved on holistic scene reconstruction, such as MonoSDF~\cite{yu2022monosdf} and ManhattanSDF~\cite{guo2022neural}, editing/manipulating 3D geometry of components from a reconstructed scene based on user instructions remains a challenging problem due to lacking semantics of the composed nature of holistic mesh}
%the composed nature of the holistic mesh without semantic information.
%which are implicitly encoded into neural network weights. 

%There have been a few attempts~\cite{wu2022object, wu2023objectsdf++, li2023rico, kong2023vmap} to explicitly decompose a scene into individual objects by using separate MLP layers to represent particular objects, which causes scalability issues if the scene contains a large number of objects. 
%Besides, their success relies heavily on human-annotated instance masks on multiview images for training, which are hard to acquire in practice.

A few attempts have been made to decompose a reconstructed 3D scene into individual objects using separate Multi-Layer Perceptron (MLP) layers to represent specific objects~\cite{wu2022object, wu2023objectsdf++, li2023rico, kong2023vmap}. However, these approaches face scalability issues when dealing with scenes containing numerous objects~\cite{kong2023vmap}. Furthermore, the success of these methods heavily relies on human-annotated instance masks on multi-view images during training, which poses challenges in obtaining them for large-scale practical applications. Moreover, even with ground-truth instance labels, the existing state-of-the-art method~\cite{wu2023objectsdf++} still fails to produce satisfactory results, with multiple objects missing, as shown by the second row of Fig.~\ref{fig: final_results}, due to the inherent difficulties in separating all objects using implicit representations.
\begin{comment}
A few attempts have been made to decompose a reconstructed 3D scene into individual objects by employing separate MLP layers for representing specific objects~\cite{wu2022object, wu2023objectsdf++, li2023rico, kong2023vmap}. 
However, this approach leads to scalability issues when handling scenes with numerous objects ~\cite{kong2023vmap}. 
Moreover, the success of these methods heavily relies on human-annotated instance masks on multi-view images for training, which are difficult to obtain for large-scale practical applications.
Even with ground-truth view-consistent instance labels, existing state-of-the-art method \cite{wu2023objectsdf++} still cannot achieve satisfying results with many objects missing, as shown in \xjqi{Fig.\ref{fig: missing structure}}, due to the difficulties of separating all objects using implicit representations. 
\end{comment}
%{Surprisingly, existing state-of-the-art, like ObjSDF++, will missing many objects even with ground truth label as shown in Fig.~\ref{fig: missing structure}}

\begin{comment}
\xjqi{still thinking about whether keep it here or move it to related work}Another line of research in decompositional neural rendering \xjqi{LERF, xxx add citations} investigates the distillation of generalized features or segmentation predictions \xjqi{add panoptic, DM-NeRF??} from large-scale pre-trained image backbones, such as DINO~\cite{caron2021emerging}, CLIP features~\cite{radford2021learning} and \xjqi{panoptic segmentation}, to neural fields. 
These approaches leverage feature similarities or predicted instance/semantic codes for grouping and implicitly decomposing a scene, requiring no additional human annotation efforts and offering greater scalability for large-scale scenes.
However, when directly applied to the reconstruction task, these strategies often produce decomposed outputs that are incomplete and exhibit poorly defined contours (see Fig. \xjqi{xxx}) due to ill-defined object boundaries \xjqi{add citations} or multiview inconsistent and low-quality segmentation predictions  \xjqi{add citation} used during training. 
\end{comment}

%, hindering the decomposition of high-quality object shapes from a scene and downstream applications. 
%However, when directly applying these strategies to the reconstruction task, the resulting decomposed outputs are often incomplete and lack well-defined contours due to poorly defined object boundaries \xjqi{add citations} or multiview inconsistent and low-quality segmentation predictions for training \xjqi{add citation}, hindering the extraction of high-quality object shapes (see \xjqi{Fig. xxx}).
%, and leverages feature similarities or predicted instance codes for grouping and implicitly decomposing a scene.
%These methods do not require additional human annotation efforts and are more scalable for large-scale scenes. 
%However, directly applying these strategies to the reconstruction task yields decomposed outputs lacking well-defined contours and may not enable the extraction of individual objects due to the lack of well-defined object boundaries \xjqi{modify this later} (see \xjqi{Fig. xxx}).




\begin{comment}
A few attempts have been made to explicitly decompose a scene into individual objects~\cite{wu2022object, wu2023objectsdf++, li2023rico, kong2023vmap} by using separate MLP layers for representing specific objects. However, this approach leads to scalability issues when dealing with scenes containing a large number of objects. Furthermore, the success of these methods heavily depends on human-annotated instance masks on multi-view images for training, which are difficult to obtain in practical large-scale applications. 
Another line of research in neural rendering explores distilling generalized features from large-scale pre-trained image backbones, such as DINO~\cite{caron2021emerging},  to neural fields and relies on feature similarities to perform grouping and implicitly decompose a scene. 
These methods don't require additional human efforts for annotation and are more scalable to large-scale scenes. 
Although they have shown promising scene editing results in neural rendering, directly applying these strategies to the reconstruction task results in decomposed outputs that lack well-defined contours and may not enable the extraction of individual objects due to the inaccuracy of features (see \xjqi{Fig.}~\ref{fig: distill features}).
\end{comment}

%There are some attempts~\cite{wu2022object, wu2023objectsdf++, li2023rico, kong2023vmap} for neural implicit surface decomposition, which heavily relies on human-annotated instance-level masks~\cite{siddiqui2022panoptic} \xjqi{the citation is not correct} or 3D detection bounding boxes~\cite{szot2021habitat} \xjqi{the citation is not correct}.
%However, it is difficult to obtain the view consistent instance-level masks or accurate 3D bounding boxes, and the granularity of decomposition is hard to be controlled.

\begin{comment}
In addition, distilling generalized features from pre-trained image backbones such as L-Seg~\cite{li2022language}, CLIP~\cite{radford2021learning}, and DINO~\cite{caron2021emerging} have been used for developing decomposed neural radiance field focusing on editing the visual effect of interested regions which will be hard for the embodied simulation.
But directly applying these strategies to the implicit SDF field~(Fig.~\ref{fig: distill features}), results in decomposition outputs that may lack well-defined contours, and may not enable the extraction of independent instance segmentation results.
\end{comment}

%In this paper, we present a new method, namely Total-Decom, tailored to decomposed 3D reconstruction with minimal human interactions. Our approach can decompose a 3D scene into independent desired components controlled by users, further allowing geometry and appearance editing of these decomposed fragments.
%In this paper, we present Total-Decom, a novel method tailored for decomposed 3D reconstruction with minimal human interaction. The core of our method is a novel integration of the Segment Anything Model (SAM), an interactive segmentation model with hybrid implicit and explicit surface representations for reconstruction, decomposition, and real-time interaction, enabling the decomposition of a scene into individual objects with only one click per object and allowing users to control the granularity for decomposition.  
%This further allows geometry and appearance editing of these decomposed fragments.

In this paper, we introduce \textit{Total-Decom}, a novel method designed for decomposed 3D reconstruction with minimal human interaction. 
At the core of our method lies the integration of the Segment Anything Model (SAM)~\cite{kirillov2023segment}-- an interactive image segmentation model--  hybrid implicit and explicit surface representation, and a mesh-based region-growing approach. 
This integration allows the decomposition of a scene into the background and individual objects 
with minimal interactions and provides users with control over the granularity and quality of decomposition via real-time interactions, as shown in Fig.~\ref{fig:teaser}.  

Specifically, our method first employs an implicit neural surface representation for its ability to achieve dense and complete 3D reconstruction from images. 
At this stage, we also integrate object-aware information by distilling image features from the SAM model for follow-up efficient interaction and accurate decomposition. 
After obtaining the learned implicit surface and features, our approach further extracts explicit mesh surfaces while distilling features into their vertices. 
The explicit representation provides valuable geometry topology information for scene decomposition and enables real-time neural rendering to enhance human interactions. 
Then, in order to identify and separate the desired object for surface decomposition, we utilize the SAM decoder and the rendered SAM feature, converting a human-annotated click on a single rendered image view into corresponding dense object masks. 
Thanks to the segmentation capability of SAM and our feature rendering design, this interactive process also allows users to obtain the desired objects at different granularities while minimizing human interactions and avoiding high computational costs.
% allows user control over the granularity and quality of desired objects 
Lastly, with the derived object mask from a single view with good object boundaries serving as object seeds, we propose a mesh-based region-growing module that progressively expands these seeds along the mesh surface to obtain decomposed 3D object surfaces. 
This process leverages distilled feature similarities of vertices and 3D mesh geometry topology for accurate object decomposition, further ensuring precision by confining the growing process to mask boundaries obtained from the SAM decoder.

%The module leverages distilled feature similarities of vertices and 3D mesh geometry topology for accurate object decomposition, further ensuring precision by confining the growing process to mask boundaries obtained from the SAM decoder.
%leveraging distilled feature similarities of vertices and 3D mesh geometry topology for accurate object decomposition, further ensuring precision by confining the growing process to mask boundaries from SAM decoder.


%Then, to identify a desired object for surface decomposition, we leverage the SAM decoder and the rendered SAM feature to convert the human click on one rendered image view into corresponding dense object masks. 
%Geometry-guided regularization with semantic priors disentangles foreground objects and backgrounds, including occluded and invisible regions. 
%Utilizing the SAM decoder, image clicks are converted into dense object masks, allowing user control over granularity and quality while minimizing human interactions and circumventing high computational costs. 
%facilitates geometry and appearance editing of these decomposed fragments. 
%, enabling the decomposition of a 3D scene into independent user-controlled components. 


%In this paper, we introduce a novel method, Total-Decom, specifically designed for decomposed 3D reconstruction with minimal human interaction. Our approach enables the decomposition of a 3D scene into independent user-controlled components, further facilitating geometry and appearance editing of these decomposed fragments. 
%The core of our method is a novel integration of the segment anything model (SAM), an interactive segmentation model, with hybrid implicit and explicit surface representations for reconstruction and decomposition of desired objects/parts with as minimal as one click. 


%The core of our method is integrating an interactive segmentation model, {\ie} the Segment Angthing Model (SAM) \xjqi{add citation}, into a neural implicit reconstruction model to allow users to select and modify the desirable objects or parts with one click.


\begin{comment}
Our method first adopts an implicit neural surface representation to achieve dense and complete 3D reconstruction from images while incorporating object-aware information by distilling image features from the SAM model into an implicit neural feature field. Importantly, we introduce geometry-guided regularization integrated with semantic priors to disentangle foreground objects and backgrounds including occluded and invisible regions.


Upon obtaining the learned implicit surface and features, our approach further extracts explicit mesh surfaces for foreground objects and background and distills features into their vertices. The explicit mesh surface provides valuable geometry topology information for follow-up scene decomposition and enables real-time neural rendering to enhance human interactions. 


Then, given rendered images and features from the mesh surface, our method employs the SAM decoder to convert image clicks into dense object masks to precisely identify the target object in one rendered view and allow users control over granularity and quality while minimizing human interactions. Notably, by leveraging the rendered SAM features from our model, we only require the decoding process of the SAM model at this stage, thus circumventing high computational costs. 

%This process allows users to add control over the granularity and quality and facilitates the transformation of sparse clicks into dense masks for precise identification of the target object and its boundaries, harnessing the SAM model's capabilities and minimizing human interactions. Notably, by leveraging the rendered SAM features from our model, we only require the decoding process of the SAM model at this stage, thus circumventing high computational costs. 


Lastly, using the vertices corresponding to dense object masks as seeds, we propose a mesh-based region-growing module that progressively expands the seeds along the mesh surface to obtain object surfaces. This module harnesses the feature similarities of vertices and the geometry topology of the 3D mesh to achieve accurate object decomposition. The growing process is also confined by the vertices corresponding to mask boundaries, which further ensures the precision of object decomposition.
\end{comment}

We extensively validate our approach on benchmark datasets. More importantly, our high-quality decomposed 3D reconstruction enables many downstream applications in manipulating and animating objects in virtual environments, including re-texturing~\cite{chen2023text2tex} with diffusion model, deformation, and motion. (See Fig.~\ref{fig:teaser} and videos in supplementary). 

In sum, our main contributions are as follows: 

%Specifically, we first employ implicit neural surface representation for dense and complete 3D reconstruction from images and distilling image features from the SAM model to encode object-aware information into implicit neural feature fields. Notably,  we inject geometry-guided regularization with semantic priors to disentangle foreground objects and backgrounds, including invisible occluded backgrounds. 
%Given the learned implicit neural fields,  our model further extracts explicit foreground and background meshes and distills features into their vertices. 
%The explicit mesh-based representation offers geometry topology information for scene decomposition and allows neural rendering in real-time for human interactions.  
%Next, upon mesh-based surface representation and rendered image features, our approach leverages the SAM decoder to turn image clicks, serving as prompts, into dense masks, allowing transforming sparse clicks into dense masks for identifying the desired object and its boundaries, leveraging the capability of the SAM model. It is worth noting that we only need to perform the decoding process of the SAM model at this stage, thanks to our feature distillation and rendering.
%Finally, with the vertices corresponding to the dense mask as seeds, we design a mesh-based region-growing method that progressively expands the mask along the mesh surface, leveraging feature similarities of vertices and the geometry topology of  3D mesh for accuracy. The growing process is also bounded by the vertices corresponding to mask boundaries, ensuring the accuracy of object decomposition. 

%which is further leveraged for obtaining accurate object meshes. 


%renders images and features in real-time with an adapted Gaussian splatting model based on the mesh \xjqi{not sure} and allows users to identify and refine one object by clicking a point on the rendered images. 



%offers two benefits:  allowing us to design an interface integrating the SAM decoder to incorporate human interactions for accurately identifying the desired objects with only one click in real-time (\xjqi{check later}) and the potential of leveraging the geometry topology, connectivity and closeness for decomposing the desired 3D object shape.  


%We augment it with the ability to separate foreground and background by leveraging geometric priors and distill features from the SAM encoder to the implicit field for encoding object-aware information. 
%Then, the learned implicit field is distilled into an explicit mesh representation for object decomposition, editing, and human interactions.  

%the implicit field into an explicit mesh representation combined with Gaussian splatting for rendering features and images and allow rendering and object geometry decomposition in real-time. More importantly, this implicit representation allows us to leverage the \xjqi{xxx} property of 3D mesh and design a mesh-based surface growing method based on SAM-decoded object masks to determine the boundary for obtaining decomposed object-wise or human-controlled high-quality shape components. 


%\xjqi{the following needs to be rewritten} Specifically, We first train an implicit neural surface reconstruction method augmented with feature rendering and background-foreground partition. 
%Then, we distill the features into meshes for interactive selection. 
%To accurately segment precise geometry structure, we develop a mesh-based surface region growing algorithm (Section~\ref{subsec: surface}). 
%Finally, to enhance the interactive experience, we have made modifications to the Gaussian Splatting~\cite{kerbl3Dgaussians} technique. 
%This adaptation allows us to render images on fixed mesh vertices, opening the door to real-time interactivity with the reconstructed mesh, encompassing its geometry and rendering aspects.

%\xjqi{looks fine, we can revise it later}
\begin{itemize}
    \item We introduce a novel pipeline that seamlessly integrates the segment anything model with hybrid implicit-explicit neural surface representations for 3D decomposed reconstruction from sparse posed images. Our approach requires minimal human annotations (approximately one click per object on average) while achieving high decomposition quality.

    %We introduce a new pipeline, integrating SAM with hybrid implicit explicit neural surface representations for 3D decomposed reconstruction from sparse posed images, requiring minimal human annotations ({around one click on average per object}) while achieving high decomposition qualities.  
   
    \item We propose a new mesh-based region-growing method that leverages the geometry topology of 3D mesh, feature similarities among vertices, object masks, and boundaries derived from the SAM model to accurately identify and extract object surfaces for decomposition. 
    
    \item We perform an extensive evaluation of our approach on various datasets, demonstrating its superior ability to decompose objects with high accuracy. Furthermore, we showcase the potential of our results for numerous downstream tasks, such as animation and scene editing.
\end{itemize}

    %Our model also has the flexibility to allow users to control the granularity of decomposition and perform editing through our user-friendly interface and efficient mesh-based neural rendering. 
% Introduction of an innovative decomposed reconstruction pipeline, achieving comprehensive 3D scene decomposition. 
    %This relies on easily obtained foreground and background segmentation masks, coupled with generalized promptable features.
 %Proposal of a neural mesh-friendly surface-growing algorithm, facilitating the selection of objects of interest from any viewpoint {with only one or two clicks}.
   % \item Design of an intuitive GUI, enabling interactive object editing directly from the neural radiance field.
% Scene decomposition has long been a subject of investigation in the fields of computer vision and computer graphics. 
% It will enhance the interaction with the desired 3D structure and visual content in order to create a more immersive virtual world and enable various applications in embodied simulation.
% Recently, neural volumetric representations such as neural radiance field (NeRF)~\cite{mildenhall2021nerf} have emerged as a compelling bridge to connect the rendering with perception and reconstruction.
% This breakthrough facilitates the integration of perceptual findings to decompose the outcomes of both reconstruction and rendering processes.
% The majority of these approaches utilize representations in the form of volume density, occupancy\cite{oechsle2021unisurf}, signed distance functions (SDF)~\cite{wang2021neus, yariv2021volume}, or hybrid variations thereof~\cite{Lyu_2023_ICCV}. 
% These representations are employed in conjunction with multilayer perceptrons (MLPs) and hash grids~\cite{mueller2022instant, yu2022monosdf} to map the input positions to the volumetric function, view-dependent emitted radiance, and semantic information~\cite{zhi2021place}.
% Subsequently, neural rendering techniques are employed to synthesize the aforementioned properties along a single ray and obtain the pixel value.

% Incorporating perceptual capabilities, neural volumetric representations have commonly delineated scenes into two distinct categories:
% (1) Object Compositional Reconstruction~\cite{wu2022object, wu2023objectsdf++, li2023rico, kong2023vmap}:
% These approaches utilize ground truth instance segmentation masks or bounding boxes to partition the holistic scene into multiple implicit fields. Subsequently, compositional functions are employed to amalgamate these fields into a unified whole. 
% Although they can obtain accurate geometry results for any instance, these techniques heavily rely on precise and detailed labeling, thereby constraining the level and quantity of decomposition.
% (2) Decomposed Scenes with Generalized Features~\cite{kobayashi2022decomposing, goel2022interactive, tschernezki2022neural, wang2023autorecon, lerf2023}:
% These methods aim to decompose the scenes with generalized features. They always distill features into volumetric representations, such as L-Seg~\cite{li2022language} features, CLIP features~\cite{radford2021learning}, and DINO~\cite{caron2021emerging} features, et al. 
% Subsequently, an attention-based selection technique is employed to identify specific visual regions after traversing the entirety of the 3D space.
% However, these approaches predominantly emphasize the quality of novel view synthesis while potentially overlooking the importance of geometric accuracy. 
% Directly applying these strategies to the implicit SDF field~(Fig.~\ref{fig: distill features}), results in decomposition outputs that may lack well-defined contours, and may not enable the extraction of independent instance segmentation results, thus significantly affecting downstream applications, such as animations.

% Therefore, this paper presents the Total-Decom framework, which is designed to reduce dependence on 2D instance segmentation masks and concurrently acquire a comprehensive and accurate representation of instance-level geometry.
% Inspired by the strengths of two leading decomposition approaches, we employ readily attainable foreground and background segmentation masks (encompassing elements such as walls, floors, and ceilings) to create a preliminary division of the scene into two distinct fields. 
% Within the foreground field, we distilled promptable generalized features, such as the Segment Anything Model feature~\cite{kirillov2023segment}, to execute meticulous and fine-grained segmentation of the entire scene.
% With this approach, we can not only enhance the quality of reconstruction for both scenes and objects but also achieve a complete decomposition of indoor scenes at an instance level.

% To accommodate the traits of promptable features and enable the direct selection of desired meshes from any viewpoint, we devised a mesh-based surface growing algorithm (Section~\ref{subsec: surface}). 
% This algorithm utilizes generalized features distilled onto mesh vertices, enabling us to acquire the precise geometric structure of any object from a single frame. 
% Notably, this approach eliminates the need for iterative rendering to obtain the 3D structure of the object, a requirement present in prior methods.
% Furthermore, to enhance the interactive experience, we have made modifications to the Gaussian Splatting~\cite{kerbl3Dgaussians} technique. 
% This adaptation allows us to render images on fixed mesh vertices, opening the door to real-time interactivity with the reconstructed mesh, encompassing both its geometry and rendering aspects.

% Overall, our main contributions are as follows.
% \begin{itemize}
%     \item We propose a new decomposed reconstruction pipeline to totally decompose a 3D scene relying on the easier obtained foreground and background segmentation masks and generalized prompotable feature.
%     \item We propose a neural mesh-friendly surface-growing algorithm that can help us to select the interested objects in any view.
%     \item We design an easy-to-use GUI to interactively edit any objects from neural radiance field. 
%     \item We evaluate our method on different datasets and demonstrate that our method can decompose more objects in a more user-friendly manner, and also show great potential with many downstream tasks like animation and scene editing.
% \end{itemize}

% Previous version & comments
% \xjqi{P1: what's the problem, why is it important. [you may emphasis interactive if needed]
% We explore the problem of decomposed 3D reconstruction and rendering [not sure whether we emphasize rendering or not??], aiming to recover the geometry of xxx and xx, from a few posed images [refer to teaser images]. This is an important research problem that enables many applications in embodied simulation, scene editing, ... }

% \xjqi{P2. 1. a general summary of existing methods for decomposition. Better categorize them into multiple streams. (stream 1: object nerf, object nerf++. [not sure whether we mention a) label space distillation?? panoptic lifting and so on. b) feature space decompostion (DINO feature) c) DM-NeRF] Summarize each stream of work and their advantages and limitations. [maybe we can focus on approaches that focus on evaluating reconstruction capability and leave other methods into the related work] 3. Motivate your solution  }


% \xjqi{P3. Your solution and pipeline 1. the first sentence to summarize your approach. 2 several sentences to describe key components of your methods and link them as a coherent story. We first put forward a feature xxxx. Then, to xxx, we xxxx. [write as we discussed]  3. analyze and summary echo why your problem address aforementioned issues (echo P2.)}

==> sec/2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}
%\xjqi{more citations should be discussed such as DM-NeRF especially their papers mentioned decomposed reconstruction}
%\vspace{0.1in}
\vspace{0.1in}\noindent\textbf{Object Compositional Reconstruction}
In order to better reconstruct the geometry of objects in complex scenes, many research efforts have been devoted to exploring better object-level compositional scene representations. For instance, ObjSDF \cite{wu2022object} proposes a compositional scene representation to assist in geometry optimization in highly composite scenes and better object-level extraction with the help of multi-view consistent instance labels. Kong {\etal} \cite{kong2023vmap} build an object-level scene model from a real-time RGB-D input stream for object-compositional SLAM. Wu {\etal} build upon ObjSDF and further mitigate object occlusions in complex scenes through an object distinction regularization term. Additionally, a new occlusion-aware object opacity rendering scheme is introduced to reduce the negative impact of occlusion on scene reconstruction. However, these methods rely heavily on accurate multi-view consistent ground-truth instance-level labels and cannot effectively preserve all objects within the reconstruction.
%limiting their downstream applications. 

\vspace{0.1in}
\noindent\textbf{Decompositional Neural Rendering} Neural radiance fields (NeRFs) offer a unified representation to represent the appearance~\cite{mildenhall2021nerf, yu2021pixelnerf}, and other spatially varying properties~\cite{Kundu_2022_CVPR}. 
In the field of decompositional neural rendering, many research efforts investigate the distillation of generalized features~\cite{lerf2023, goel2022interactive, kobayashi2022decomposing,tschernezki2022neural}, or segmentation predictions~\cite{siddiqui2022panoptic, bing2022dm} from large-scale pre-trained image backbones, such as DINO~\cite{caron2021emerging, oquab2023dinov2}, CLIP features~\cite{radford2021learning} and panoptic segmentation~\cite{cheng2022masked}, to neural fields. 
Specifically, Semantic NeRF \cite{zhi2021place} explores incorporating regressing semantic labels into the process of Novel View Synthesis.
Building upon this, distilled feature fields (DFFs) \cite{kobayashi2022decomposing} and neural feature fusion fields (N3F) \cite{tschernezki2022neural} have emerged as pioneering approaches for distilling \cite{hinton2015distilling} semantic features from pretrained models, such as LSeg \cite{li2022language} and DINO \cite{caron2021emerging}, into NeRF for decomposition. 
ISRF \cite{goel2022interactive} does not rely solely on feature matching, but instead obtains the final results through region growing.
These approaches leverage feature similarities or predicted instance/semantic codes for grouping and implicitly decomposing a scene, requiring no additional human annotation efforts and offering greater scalability for large-scale scenes.  However, when directly applied to the reconstruction task, these strategies often produce decomposed outputs that are incomplete and exhibit poorly defined contours (see Fig.~\ref{fig: selected_mesh}) due to ill-defined object boundaries~\cite{goel2022interactive} or multiview inconsistent and low-quality segmentation predictions~\cite{wang2022dm, cheng2022masked, he2017mask} used during training. 
In contrast to existing methods, our work not only avoids the need for extensive manual interaction through a geometry-guided feature approach but also enables the extraction of any constituent part of a complex scene.
% No feature distillation
%Another line of research, such as NeRFshop \cite{jambon2023nerfshop}, utilizes geometric cues for object selection in a scene. However, the lack of object awareness often leads to unstable object segmentation in a complex scene. 
%Based on existing methods, users either cannot completely decompose the scene or need to rely on extensive interactions to achieve the goal of decomposing the scene, contradicting the initial design intention of labor-saving. 

% Promptable feature
%\vspace{0.1in}
\vspace{0.1in}\noindent \textbf{NeRF with SAM} SAM~\cite{kirillov2023segment} achieves efficient 2D interactive segmentation capabilities through extensive high-quality annotated supervision. 
It brings forth more possibilities in this field and has the potential to help achieve thorough decomposition of complex scenes with plausible 2D segmentation capabilities. Recently, some concurrent works have explored the combination of SAM and NeRF for decomposition.
SA3D~\cite{cen2023segment} incorporates cross-view self-prompting technique to obtain multi-view consistent masks. However, running SAM multiple times incurs high computational costs, and the segmentation results are sensitive to interaction trajectories, leading to unstable performance.
%In this work, we incorporate SAM into our reconstruction pipeline via feature distillation, utilizing its lightweight decoder to generate dense object seeds based on rendered features for decomposition according to user-provided clicks.

% Focus on 3D representaion
%Existing research has devoted significant efforts to decomposition in terms of visual rendering, but extracting the constituent parts as fundamental 3D representations, such as mesh, from the scene still remains an underexplored area with limited research.
%AutoRecon \cite{wang2023autorecon} enables reconstructing the main objects in a scene in n a decompositional manner, but it is specifically designed for object-centric scenes.
% Conclude about our work
%In contrast to existing methods, our work not only avoids the need for extensive manual interaction through a geometry-guided feature approach but also enables the extraction of any constituent part of a complex scene.
%\xjqi{mention SAM and NeRF combination works}




==> sec/3_method.tex <==
\section{Empirical Study on General Visual Features}
\label{sec:features}

\begin{figure}[t]
% \vspace{-10pt}
    \centering
    \includegraphics[width=\linewidth]{./figure/PCA.pdf}
    \vspace{-15pt}
    \caption{Visualization for distilled generalized features.}
    \label{fig: feature study}
    \vspace{-10pt}
\end{figure}

\begin{figure}[t]
% \vspace{-10pt}
    \centering
    \includegraphics[width=\linewidth]{./figure/selected_mesh.pdf}
    \vspace{-15pt}
    \caption{Comparison on different decomposition methods with SAM feature. SAM + region growing represents object extraction with our method. SAM + similarity indicates object extraction with similarity matching in 3D space, following \cite{tschernezki2022neural, kobayashi2022decomposing}.}
    \label{fig: selected_mesh}
    \vspace{-12pt}
\end{figure}

\begin{figure}[htb]
\begin{center}
  \includegraphics[width=1.0\linewidth]{figure/feat.pdf}
  \vspace{-15pt}
  \caption{Visualization of the SAM feature for the same object in different views with t-SNE~\cite{JMLR:v9:vandermaaten08a}.
  All the features are in the same feature space.}
  \vspace{-20pt}
  \label{fig: tsne}
\end{center}
\end{figure}

%Decomposed 3D scene reconstruction requires object-aware knowledge to separate individual objects and the background. 
%reconstruction is how to inject s into a 3D scene. 
A central challenge in decomposed 3D scene reconstruction is incorporating object-aware knowledge to accurately separate individual objects and backgrounds. While existing methods have explored the use of ground-truth multi-view consistent instance-level annotations~\cite{wu2022object, wu2023objectsdf++, li2023rico, kong2023vmap}, these approaches suffer from high annotation costs and scalability issues. Motivated by recent advancements in vision foundation models providing generic features, we investigate their potential for object decomposition and reducing human annotation requirements. Although this strategy has been examined in neural rendering~\cite{kobayashi2022decomposing,goel2022interactive,tschernezki2022neural}, it remains under-explored in decomposed 3D reconstruction, which necessitates more precise boundary information. Accordingly, we investigate features from three foundation models: CLIP-LSeg \cite{li2022language}, DINO \cite{caron2021emerging}, and SAM \cite{kirillov2023segment}.
\begin{comment}
A central question to decomposed 3D scene reconstructions is how to inject accurate object-aware knowledge that can be used to separate individual objects and backgrounds. 
Although existing methods have explored using ground-truth multi-view consistent instance-level annotations to inject such information ~\cite{wu2022object, wu2023objectsdf++, li2023rico, kong2023vmap}, this strategy, however, suffers from high annotation costs and scalability issues. 
Motivated by the recent advancements of vision foundation models that provide generic features, we investigate whether they can be utilized for object decomposition and reduce the requirement of human annotations. 
Although this strategy has been investigated in neural rendering \xjqi{add citations}, this is still under-explored in decomposed 3D reconstruction,  which requires more accurate boundary information. 
We thus investigate features from three foundation models: CLIP-LSeg \cite{li2022language}, DINO \cite{caron2021emerging}, and SAM \cite{kirillov2023segment}. 
\end{comment}

We utilize the MonoSDF~\cite{yu2022monosdf} for implicit neural surface reconstruction, augment it with a feature rendering head, and distill features from the above 2D backbones. The rendered features after distillation are depicted in Fig.~\ref{fig: feature study}. We observe that: (1) distilled CLIP-LSeg features cannot distinguish objects of the same categories; (2) distilled DINO features lack accurate object boundaries; and (3) distilled SAM features preserve object boundaries. However, none of these features are discriminative enough to accurately separate different object instances. For example, while SAM features perform the best, directly grouping 3D objects based on similar feature responses leads to the merging of distant areas due to the absence of geometry and object boundary information, as shown in Fig.~\ref{fig: selected_mesh}.
%For example, while SAM features perform the best, highlighted areas exhibit similar feature responses and grouping 3D objects based on features as shown in Fig. \ref{fig: selected_mesh} \xjqi{combines distant areas due to the lack of geometry and object boundary information}. 


Despite the above shortcomings, we observe that the distillation brings the features of the same object from different views closer than the original 2D features from SAM, suggesting that high feature similarity often indicates a high likelihood of belonging to the same object, as shown in Fig.~\ref{fig: tsne}. 
Consequently, we propose a novel approach that leverages SAM features and a mesh-based region-growing method to decompose a 3D scene with minimal human annotations, typically requiring only one click per object.


%Despite the above shortcomings, we observe that the distilled features make the features of the same object from different views closer than the original 2D features from the SAM features, indicating that the high feature similarity often indicates a high possibility of belonging to the same object. 
%Thus, we propose combining with an explicit representation, {\ie} mesh, allowing the model to leverage geometry for object decomposition, and design a mesh-based region-growing method that progressively expands to obtain an object with seeds and boundary information from masks obtained using the SAM decoder. Our final results are illustrated in \xjqi{Fig. xxx}.
%. This indicates points of features with a high similarity tend to be the same object if they are spatially close in 3D (see Fig. xx). 

\begin{comment}
We employ the \xjqi{xxx[which method you use]} for implicit neural surface reconstruction, augment it with a feature rendering head, and distill features from these 2D backbone encoders to train it.   The rendered features after distillations are shown in  Figure~\ref{fig: feature study}.  
We find that: 1) the distilled CLIP-LSeg features cannot distinguish objects of the same categories, 2) the distilled DINO features lack accurate object boundaries, and 3) the distilled SAM features preserve object boundaries. 
Besides, they are all not discriminative enough to be directly used to separate different object instances at high accuracy.  For instance, although the SAM features perform the best,  the highlighted areas have similar feature responses \xjqi{add}, and grouped 3D objects based on features are shown in \xjqi{Fig.}: group far-away areas together \xjqi{add descriptions later} due to the lack of geometry information and object boundary information. 
The above motivates us to employ an explicit representation to allow the model to leverage geometry information for object decomposition and design a mesh-based region-growing method with initialization and boundary information from masks obtained from the SAM decoder.  Our final results are illustrated in \xjqi{Fig. xxx}.  
%Despite the challenges, we find that features of the same object are 
\end{comment}


%Among them, the distilled features from SAM are the most suitable for decomposition. 
%We directly performing grouping cannot yield high-quality 3D decomposed objects as shown in \xjqi{Fig. x}: \xjqi{add descriptions later}. 
%Further, we explore a naive solution to decompose different objects by grouping them based on the similarities of distilled features and extracting corresponding 3D objects. The results shown in Fig. \xjqi{??} demonstrate that the 




\begin{comment}
CLIP-LSeg features capture semantic information rather than instance-level details, making it difficult to separate different instances with the same semantics.
In addition, CLIP feature comparison across the entire 3D space are highly sensitive to similarity thresholds and inevitably introduce noise.
An example is illustrated in Figure~\ref{fig: selected_mesh}.
DINO features struggle to accurately represent complex scenes, as the semantics of objects from different viewpoints cannot be guaranteed, necessitating the reliance on viewpoint switching and heavy user interaction to obtain the 3D structure of objects \cite{goel2022interactive}.
In addition, the unclear boundaries between foreground objects in DINO feature further restricts the potential of using DINO feature to demarcate complex scenes.
Distilled SAM features, which have a natural alignment with the mask decoder, possess clear boundaries at the object-level and even the part-level, enabling a deeper extraction of information in the 2D space. 
The precise alignment between 2D pixel-level masks and 3D point-level features opens up possibilities for extracting 3D object information from a single viewpoint.
\end{comment}



%The advancements in 2D foundation models with superior object understanding abilities have motivated researchers to distill features from 2D foundation models into a 3D neural feature field \cite{kobayashi2022decomposing, goel2022interactive, tschernezki2022neural} and leverage them to perform decomposition implicitly through comparing feature similarities \xjqi{add citation}.  The distillation process will enforce learning 3D consistent features from 2D features that may exhibit inconsistencies across different views. 
%Despite advancements, these investigations are mainly conducted to enhance neural rendering, which does not necessarily require accurate surface reconstructions.   

\begin{comment}
Object-level semantics are crucial for decomposing a reconstructed scene, especially for separating objects with tightly adjacent geometric structures, such as adjacent pillows. 
Many vision foundation models \cite{kirillov2023segment,caron2021emerging,li2022language} have demonstrated their plausible generalization capabilities in extracting objectness in 2D images.
Existing methods \cite{kobayashi2022decomposing, goel2022interactive, tschernezki2022neural} have demonstrated the promising potential of leveraging capabilities from 2D image-based networks for 3D segmentation, bridged by neural implicit representation.
Distilling the 2D features with additional neural field, adopted by these work, helps transfer the attributes of 2D features to 3D representations.
A crucial challenge in achieving a complete decomposition of the scene lies in finding appropriate 2D features for guidance, which remains inadequately studied.
To address this, we study the features from the main-stream feature extractors: CLIP-LSeg\cite{li2022language}, DINO\cite{caron2021emerging} and SAM\cite{kirillov2023segment}.


% Feature study figure:
% Format: Ori v.s. Distilled v.s. SAM v.s. distilled SAM
% LSeg visualization: instance
% DINO: wall dirty vis
% Mesh extraction results, In total 3x4
As shown in Figure~\ref{fig: feature study}, CLIP-LSeg features capture semantic information rather than instance-level details, making it difficult to separate different instances with the same semantics.
In addition, CLIP feature comparison across the entire 3D space are highly sensitive to similarity thresholds and inevitably introduce noise.
An example is illustrated in Figure~\ref{fig: selected_mesh}.
DINO features struggle to accurately represent complex scenes, as the semantics of objects from different viewpoints cannot be guaranteed, necessitating the reliance on viewpoint switching and heavy user interaction to obtain the 3D structure of objects \cite{goel2022interactive}.
In addition, the unclear boundaries between foreground objects in DINO feature further restricts the potential of using DINO feature to demarcate complex scenes.
Distilled SAM features, which have a natural alignment with the mask decoder, possess clear boundaries at the object-level and even the part-level, enabling a deeper extraction of information in the 2D space. 
The precise alignment between 2D pixel-level masks and 3D point-level features opens up possibilities for extracting 3D object information from a single viewpoint.
\end{comment}

\begin{figure*}
% \stepcounter{figure}
  \centering
    % \centering
        \includegraphics[width=0.98\linewidth]{./figure/pipeline_v3.pdf}
    %     \vspace{-18pt}
    % \vspace{6pt}
    \caption{\textbf{Overview of \textit{Total-Decom}.} (1) \textbf{Foreground and background decomposed neural reconstruction.} 
    We have four networks in this stage to predict the geometry, appearance, semantic, and SAM features per point.
    We follow the ObjSDF++~\cite{wu2023objectsdf++} to use the foreground and background compositional representation with pseudo geometry priors and apply $\min$ operation to construct the whole scene.
    Notably, the foreground is constrained with object distinct loss (Eq.~\eqref{eq: obj_distinct}) and the background is regularized with Manhattan loss (Eq.~\eqref{eq: manhattan}) and floor reflection loss (Eq.~\eqref{eq: floor}).
    Furthermore, we also train a solely feature network to render the generalized features.
    (2) \textbf{Interactive Decomposition.} We firstly extract the  SAM feature from the feature network into the vertices of the reconstruction mesh.
    Subsequently, for any given pose, we can render a color image and a feature image.
    Passing the feature image and user-selected prompt into the SAM decoder allows us to obtain the 2D mask of the regions of interest. 
    Utilizing our newly proposed surface region-growing algorithm, we can then acquire the 3D mesh corresponding to these regions.
    Our method enables the user to select objects with varying levels of granularity, requiring just one or two clicks.
    }
    \label{fig: pipeline} 
    \vspace{-6pt}
\end{figure*}
\section{Overview}
\label{sec:overview}

Our objective is to reconstruct a 3D scene from multi-view images and decompose it into individual object entities and the background while minimizing the need for human annotations. To achieve this, we propose a novel pipeline that integrates SAM into a hybrid implicit-explicit surface representation, combined with a mesh-based region-growing method to effectively identify and decompose arbitrary 3D objects within a scene. The overview of our approach is illustrated in Fig.~\ref{fig: pipeline}.

As shown in Fig.~\ref{fig: pipeline} (Left) and detailed in Sec. \ref{sec:neural_implicit_feature_distillation_and_reconstruction}, we first adopt an implicit neural surface representation to achieve dense and complete 3D reconstruction from images while incorporating object-aware information by distilling image features from the SAM model into an implicit neural feature field (see Fig.~\ref{fig: pipeline}: bottom ). 
Importantly, we introduce geometry-guided regularization integrated with semantic priors to disentangle foreground objects and backgrounds, including occluded and invisible background regions with details unfolded in Sec.~\ref{sec:neural_implicit_feature_distillation_and_reconstruction}. 


Upon obtaining the learned implicit surface and features, our approach further extracts explicit mesh surfaces for foreground objects and background; see Fig. ~\ref{fig: pipeline}: Background $d_B(p)$ and Foreground $d_F(p)$; and distills features into their vertices; see Fig.~\ref{fig: pipeline}: Neural Mesh. 
The explicit mesh surface provides valuable geometry topology information for follow-up scene decomposition and enables real-time neural rendering to enhance human interactions. 
Then, given rendered images and features from the mesh surface, our method employs the SAM decoder to convert image clicks into dense object masks to precisely identify the target object in one rendered view (see Fig.~\ref{fig: pipeline}: Interactive Decomposition ) and allow users control over granularity and quality while minimizing human interactions.  Details are elaborated in Sec.~\ref{decomposition_with_human_interactions}. 
Notably, by leveraging the rendered SAM features from our model, we only require the decoding process of the SAM model at this stage, thus circumventing high computational costs. 

%This process allows users to add control over the granularity and quality and facilitates the transformation of sparse clicks into dense masks for precise identification of the target object and its boundaries, harnessing the SAM model's capabilities and minimizing human interactions. Notably, by leveraging the rendered SAM features from our model, we only require the decoding process of the SAM model at this stage, thus circumventing high computational costs. 

Lastly, using the vertices corresponding to dense object masks as seeds, we propose a mesh-based region-growing module that progressively expands the seeds along the mesh surface to obtain object surfaces as detailed in Sec.~\ref{decomposition_with_human_interactions}. 
This module harnesses the feature similarities of vertices and the geometry topology of the 3D mesh to achieve accurate object decomposition. 
The growing process is also confined by the vertices corresponding to mask boundaries, which further ensures the precision of object decomposition.



% \xjqi{Pleaser merge with what I have written and rewrite...}
% Our primary objective is to achieve a comprehensive decomposition (at any granularity) and facilitate the editing of the reconstructed mesh through a user-friendly interactive method.
% Initially, we employ machine-generated foreground and background segmentation masks to automatically reconstruct an indoor scene into two distinct fields. 
% This process involves applying the object distinct loss and unobserved Manhattan loss, resulting in a pure foreground mesh (Figure~\ref{fig: fg_mesh}) and a completely clean background mesh (Figure~\ref{fig: bg_mesh}).
% Concurrently, we distill generalized features, such as the Segment Anything Model features, onto the vertices of the two field meshes. 
% Following this, we introduce a novel graphic interactive application that leverages the vertices of the holistic reconstructed mesh as fixed points for fitting 3D Gaussians~\cite{kerbl3Dgaussians}, enabling real-time image rendering.
% The integration of distillation features and SAM decoder into our newly designed surface-based region-growing algorithm allows for the seamless selection of any objects or parts from any viewpoint with just one click.
% Moreover, the Total-Decom pipeline extends its support to various downstream applications, including interacting with objects (Figure~\ref{fig: application}), cross-scene editing (Figure~\ref{fig: application}), room re-texturing (Figure~\ref{fig: application})\etal.

\section{Neural Implicit Feature Distillation and Surface Reconstruction}
\label{sec:neural_implicit_feature_distillation_and_reconstruction}

In this stage, we employ an implicit neural field for reconstruction from posed images, disentangle foreground and background using geometric priors, and distill features from the SAM encoder to incorporate object-aware information. 
An illustration of our implicit reconstruction is depicted in Fig.~\ref{fig: pipeline}. 
In the following, we first elaborate on our reconstruction network and rendering formula, and then detail our core design for achieving background and foreground separation while reconstructing occluded foreground areas.

\begin{comment}
In this stage, we utilize an implicit neural field for reconstruction from posed multi-view images, disentangle foreground and background using geometric and semantic priors, and distill features from the SAM encoder to incorporate object-aware information. 
An illustration of our implicit reconstruction network, which includes a geometry MLP, semantic MLP, appearance MLP, and feature MLP, is depicted in Fig~\ref{fig: pipeline}. Specifically, the geometry MLP comprises two output heads for predicting the SDF values of foreground and background separately, where the foreground and background information is derived from the output of the semantic MLP. The appearance MLP is utilized to output RGB color given a querying point. The feature MLP is employed to render features, which are trained by distilling features from the SAM encoder. In the following, we first provide an overview of the SDF-based neural implicit surface representation and then detail our core design for achieving background and foreground separation while reconstructing occluded foreground areas.
\end{comment}

%In this stage, we employ an implicit neural field for reconstruction from a posed multiview image, disentangle foreground and background leveraging geometric priors, and distill features from the SAM encoder to inject object-aware information. An illustration of our implicit reconstruction is shown in Fig.~\ref{fig: pipeline}. 


\begin{comment}
In this stage, we want to use segment masks, posed images, pseudo geometry priors, and SAM features to reconstruct the surfaces.
Notably, the stage will automatically decompose the scene into complete foreground and background.
To achieve this goal, our neural implicit reconstruction mainly have four different networks, like the description shown in Fig.~\ref{fig: pipeline}.
% automatically decompose the whole room into two meshes, one is the pure foreground mesh and another is the complete and pure background mesh.
\end{comment}

\vspace{0.1in}\noindent\textbf{Reconstruction network and SDF-based neural implicit surface representation.}
We use the signed distance function $d(\mathbf{p})$ to represent the geometry of the surface at each point $\mathbf{p}$.
Considering a ray $\mathbf{r}(t) = \mathbf{o} + t \mathbf{v}$ from a camera position $\mathbf{o}$ in the direction of $v$, we calculate the signed distance function of each sampled point $\mathbf{p}$ using the geometry MLP and use three MLPs to predict the color $C(\mathbf{p}, v)$, semantic logits $S(\mathbf{p})$, and generalized feature $F(\mathbf{p})$ distilled from the SAM encoder, respectively; refer to Fig. \ref{fig: pipeline} for details. 
To apply the volume rendering formula, we follow VolSDF~\cite{yariv2021volume} to convert the signed distance function to volume density $\sigma(\mathbf{p})$:
\begin{equation}
    \sigma(\mathbf{p})= \begin{cases}\frac{1}{2 \beta} \exp \left(\frac{-d(\mathbf{p})}{\beta}\right) & \text { if } d(\mathbf{p}) \geq 0 \\ \frac{1}{\beta}-\frac{1}{2 \beta} \exp \left(\frac{d(\mathbf{p})}{\beta}\right) & \text { if } d(\mathbf{p})<0\end{cases},
\end{equation}
where $\beta > 0$ is a learnable parameter to decide the sharpness of the surface density. 
Then, we use the volume rendering formula~\cite{kajiya1984ray} to obtain outputs $\mathbf{E}$ of the target pixel,
\begin{equation}
    \hat{\mathbf{E}}(r) = \sum_{i=1}^{M}T^r_i\alpha_i\hat{e}^r_i \;,
\end{equation}
where $\hat{e}\in\{\hat{c}, \hat{n}, \hat{d}, \hat{s}, \hat{f}\}$ represent the predicted color, normal, depth, semantic logits, generalized feature.
$T^r_i$ and $\alpha_i$ represent the transmittance and alpha value (a.k.a opacity) of the sample point, 
and their values can be computed by
\begin{equation}
        T^r_i = \prod_{j=1}^{i-1}(1-\alpha_i), ~
    \alpha_i = 1 - \exp(-\sigma^r_i\delta^r_i) \;,
\end{equation}
where $\delta^r_i$ is the distance between adjacent sample points.

We follow the loss function $\mathcal{L}_\text{rgb}$ and $\mathcal{L}_\text{geo}$ in MonoSDF~\cite{yu2022monosdf} to optimize the rendered color, depth, and normal.
For the rendered semantic $\hat{S}(r)$, we use the cross-entropy loss defined as
\begin{equation}
    \mathcal{L}_\text{sem}=-\mathbb{E}_{\mathbf{r} \in \mathcal{R}}\left[ \sum_{l=1}^L{P}_l(r) \log \hat{P}_l({r})\right] \;,
\end{equation}
where $P_l(r), \hat{P}_l(r)$ are the multi-class semantic probability as class $l$ of the ground truth map and rendering map for ray $r$, respectively. 
Additionally, we use the $L2$ loss $\mathcal{L}_{f}$ to optimize the rendered generalized feature $\hat{F}(r)$ for distilling the $F(r)$ from the SAM encoder.


\vspace{0.1in}\noindent\textbf{Modeling foreground and background compositional scene geometry.}
To represent foreground and background geometry separately, we construct two different SDF fields $\mathcal{S}=\{\mathcal{F}, \mathcal{B}\}$ following ~\cite{wu2023objectsdf++}.
The single scene $\Omega$ is the composition of the $\Omega = \mathcal{F} \bigcup \mathcal{B}$.
The scene SDF can be calculated as the minimum of two fields SDFs $d_\Omega(\mathbf{p})=\text{min}\{d_\mathcal{F}(\mathbf{p}), d_\mathcal{B}(\mathbf{p})\}$.
To learn the geometry from the supervision of foreground and background masks, we adopt occlusion-aware opacity rendering~\cite{wu2023objectsdf++} to guide the learning of different field surfaces.
The loss function is defined as:
\begin{equation}
    \mathcal{L}_O=\mathbb{E}_{\mathbf{r} \in \mathcal{R}}[\sum_{\mathcal{S}_i \in \mathcal{S}}\left\|\hat{O}_{\mathcal{S}_i}(\mathbf{r})-O_{\mathcal{S}_i}(\mathbf{r})\right\|], 
    \label{eq: occ_aware}
\end{equation}
where $\hat{O}(r)=\int_{t_n}^{t_f} T(\mathbf{r}(t)) \alpha(\mathbf{r}(t)) d t$ to formulate the occlusion-aware object opacity in the depth range $[t_n, t_f]$.

For reconstructing the clean foreground mesh, we follow the object distinction regularization term~\cite{wu2023objectsdf++} forcing each point in a single scene to be only located inside one field, which is defined as follows: 
\begin{equation}
    \mathcal{L}_\text{reg}=\mathbb{E}_{\mathbf{p}}[\sum_{d_{\mathcal{S}_i}(\mathbf{p}) \neq d_{\Omega}(\mathbf{p})} \operatorname{ReLU}\left(-d_{\mathcal{S}_i}(\mathbf{p})-d_{\Omega}(\mathbf{p})\right)]\;,
    \label{eq: obj_distinct}
\end{equation}

Compared with the foreground, the background is more difficult to reconstruct because it has many occluded areas that are not visible in all captured views. 
%Thus, the geometric shape of the original background field is irregular, with numerous floating points.
To regularize the reconstruction of these areas, we follow the Manhattan world assumption~\cite{Yuille1999Man, guo2022neural}, i.e., the surfaces of man-made scenes should be aligned with three dominant directions.
%We can integrate it into the learning of the unobserved regions in the background field, which is defined as 
We use this to regularize the reconstruction of the floor and the wall using, 
\begin{equation}
\begin{aligned}
    \mathcal{L}_\text{man} = &\mathbb{E}_{r\in\mathfrak{F}}(\hat{p}_f(r)|1-\hat{\mathbf{n}}({r}) \cdot \mathbf{n}_f|) + \\ &\mathbb{E}_{r\in\mathfrak{W}}(\min _{i \in\{-1,0,1\}}\hat{p}_w(r)|i-\hat{\mathbf{n}}({r}) \cdot \mathbf{n}_w|),
\end{aligned}
\label{eq: manhattan}
\end{equation}
where $\hat{p}_f, \hat{p}_w$ represent the probabilities of the pixel being floor and wall derived from the semantic MLP, $\mathfrak{F}, \mathfrak {W}$ are the sets of camera rays of image pixels that are labeled as floor and wall regions, $\hat{n}_r$ is the rendering normal of rays $r$, $n_f = \left<0, 0, 1\right>$ represent the assumed normal direction in the floor regions and $n_w$ is a learnable normal to represent the normal direction in the wall regions.

\begin{figure}[t]
% \vspace{-10pt}
  \centering
    \begin{minipage}[c]{\linewidth}
        \includegraphics[width=\linewidth]{./figure/Manhattan.pdf}
    \end{minipage}
    \vspace{-10pt}
    \caption{The effect of different constraint on Replica \textit{room\_1}.}
    \label{fig: manhattan}
    \vspace{-12pt}
\end{figure}

As shown in Fig.~\ref{fig: manhattan},  applying this constraint to regularize background reconstruction will yield more regular geometry but there still exist many undesired structures due to the inaccurate semantic information of these invisible regions.
Fortunately, the majority of occlusions occur on the ground, and the ceiling corresponds one-to-one with the structure of the floor. Therefore, we can utilize the structural information of the ceiling to constrain the unknown areas on the ground.
Specifically, when we have a frame of an image that observes the ceiling, we can start from points on the ceiling $\mathbf{p}_c$, emitting a ray along the direction of gravity $\mathbf{n}_g = \left<0, 0, -1\right>$. 
In the background domain, the first point $\mathbf{p}_f$ hit by this ray is considered as the ground. 
By employing the root finding method~\cite{oechsle2021unisurf}, we locate this point and constrain its normal vector by
\begin{equation}
    \mathcal{L}_\text{floor} = | 1 - \mathbf{n}(\mathbf{p}_f)\cdot \mathbf{n}_f |.
    \label{eq: floor}
\end{equation}
As shown in Fig.~\ref{fig: manhattan}, this constraint can help us get the complete and regular background.


\section{Interactive Decomposition} 
\label{decomposition_with_human_interactions}
% \begin{figure}[t]
% % \vspace{-10pt}
%   \centering
%     \begin{minipage}[c]{\linewidth}
%         \includegraphics[width=\linewidth]{./figure/grow.pdf}
%     \end{minipage}
%     \vspace{-10pt}
%     \caption{Visualization for growing process.}
%     \label{fig: grow_vis}
%     \vspace{-12pt}
% \end{figure}
% Claim the focus in this subsection
%
%In this stage, the goal is to decompose the foreground into individual objects with minimal human interactions. 
%To begin with, we extract explicit foreground meshes from the implicit surface  
%extracted from the reconstructed implicit neural surface field and distill features to the vertices of meshes to yield the neural mesh as shown in Fig. \ref{fig: pipeline}. 
%The explicit surface allows us to leverage geometry topology and spatial connectivity information to mitigate the imperfect neural features for object decompostion.  
% Sketch our idea
%
%Different from the approaches of object-compositional representations~\cite{kong2023vmap,wu2022object,wu2023objectsdf++}, which reconstruct the scene modeling multiple SDF fields following human annotated instance labels, 
% Preview
%
%In this stage, we focus on decomposing a reconstructed scene into individual objects controlled by users. 

Upon obtaining the implicit foreground surface $d_{\mathcal{F}}$ and features, we focus on decomposing the foreground into individual objects and allowing users to control the decomposition through interactions in this stage, as shown in Fig.~\ref{fig: pipeline}. 
We propose to use an explicit mesh surface as it can provide geometry information for better decomposition and allow efficient rendering by using rasterization or combining with Gaussian splatting. We provide details on the integration of Gaussian splatting in the supplementary material.  
Hence, before conducting decomposition, we extract foreground mesh $\mathcal{M}_{\mathcal{F}}$ and distill features to its vertices $\mathcal{V} = \{v_1,...,v_n\}$. 
Then, each vertex $v_i$ is associated with a distilled feature $f_{v_i}$ and a 3D location $p_i$.  
The vertices on the mesh are connected via edges $\mathcal{E}$, which are determined by the geometry topology of the mesh. 
As shown in Sec.~\ref{sec:features}, it is still challenging to rely solely on distilled features $f_{v_i}$ to decompose 3D objects. 
Thus, we introduce human annotations to identify each object and aim to minimize human interactions. 
The following details how we realize object decomposition based on a designed mesh-based region-growing method with human interactions using our designed method. 
We will first introduce how we obtain seed points for an object by combining SAM, rendered features, and human clicks. Then we elaborate on our new mesh-based region-growing algorithm for acquiring object-level meshes to realize a complete decomposition. 

%In the following, we elaborate on how we leverage SAM to obtain a set of object seeds requiring only one click per object in most cases  in Sec.~\ref{subsec:seeds generation}, and a novel neural surface region growing algorithm for acquiring the 3D geometry in Sec.~\ref{subsec: surface}. 
% 1. representation. mesh vertex?? Render features, Gaussian splatting
% Give the whole picture of the pipeline and make the logic clear
 %We extract the foreground mesh from implicit reconstructions and distill features to its vertices. 
%Our core idea is to achieve total decomposition through a novel region-growing algorithm applied on an explicit mesh surface where the seeds are obtained through interaction and SAM decoding. 
\paragraph{Object Seed Generation}
% \label{subsec:seeds generation}

Given a $\mathcal{M}_\mathcal{F}$, the goal is to obtain a set of initial seed points for each object $o$ by using human annotations. 
As shown in Fig. \ref{fig: pipeline}, with one image  $I$ containing $o$ with corresponding feature map $f_I$  rendered from $\mathcal{M}$, the user will produce a click $c$ on the image identifying the desired object.  
Based on the click $c$, serving as the prompt, and $f_I$, a 2D mask $m_o$ that describes the object can be efficiently obtained through the lightweight mask decoder of SAM. Users are also allowed to adjust its clicks according to $m_o$ to refine it. Our experiment shows that most of the objects' mask $m_o$ can be obtained with just one click. 
The pixels in mask $m_o$ are then mapped to their corresponding vertices to yield the 3D object seeds denoted as $\mathcal{S}_o$ for the follow-up region-growing algorithm. 
This process efficiently turns a single click into a set of vertices to enhance the accuracy of identifying object $o$. 
Besides, to locate object boundaries, we also extract the contour pixels $c_o$ of $m_o$ and map them to their corresponding vertices $\mathcal{B}_o$, which forms the boundary condition for region growing. 

\begin{comment}
The pipeline of selection is shown in figure~\ref{fig: pipeline}. 
% What we need is the followng:
% 1.) rendering image
% 2.) 2D-3D pixel-point relationship (depth projection / rasterization)
% 3.) Scene layout under specific view (rendering / rasterization)
% 4.) rendering feature
% 5.） reconstructed foreground mesh with features of each vertex
Based on neural implicit feature distillation and reconstruction introduced in Sec.~\ref{sec:neural_implicit_feature_distillation_and_reconstruction}, our selection procedure involves four types of inputs: 1.) the reconstructed foreground mesh, 2.) rendered images from arbitrary views provided for user interaction, 3.) rendered features for the mesh in a vertex-centric manner, and rendered features for the corresponding view in a 2D mask-decoder friendly manner, and 4.) the delineation of foreground-background layout and the correspondence between 2D pixels and 3D vertices in the corresponding viewpoint obtained through rasterization.
The pipeline can be illustrated as follows: 
Firstly, users can prompt on the 2D rendering image according to the position of the desired object. 
Based on the prompt and the rendered features under the current viewpoint, a 2D mask that describes the object can be efficiently obtained through the lightweight mask decoder of SAM. 
Next, we can obtain the contour of the selected object under this viewpoint. 
With the relationship between pixels and vertices, we can obtain the vertices corresponding to the pixels within the object's mask as seed vertices, and the vertices corresponding to the pixels within the contour mask as growth boundaries. 
Finally, we can use the region growing algorithm introduced in Sec.\ref{subsec: surface} to obtain the mesh of the selected object.
\end{comment}

\paragraph{Region-growing on Mesh for Decompostion}
% \label{subsec: surface}
% Point out the main difference between ours and others for this specific method: we use growing algorithm on the explicit 3D representation instead of the implicit one.
%Unlike previous methods ~\cite{jambon2023nerfshop, kobayashi2022decomposing, goel2022interactive,tschernezki2022neural} that primarily focus on object extraction for novel view, our work aims to further extract the selected objects in an explicit 3D representation form, i.e., mesh.
% How to directly obtain 3D mesh with one click?
% A quick scratch about surface growing algorithm.
Given the seeds $\mathcal{S}_o$ and boundary condition $\mathcal{B}_o$, we design a region-growing method to obtain the corresponding mesh $M_o$ for object $o$.
As illustrated in Algorithm~\ref{surface_growing_alg}, the seeds $\mathcal{S}_o$ are progressively expanded along the mesh $\mathcal{M}_\mathcal{F}$ to include their connected neighboring vertices with high feature similarities.  The boundary vertices $\mathcal{B}_o$ constrain the propagation process by enforcing it to stop if including vertices that will be outside of mask $m_o$. This helps ensure the boundary accuracy of the decomposed object. 
It is worth mentioning that the geometric relationship between vertices is leveraged in this progressive expanding process, benefiting the extraction of objects and reducing computation. 
Compared to region-growing algorithm that purely relies on spatial location~\cite{goel2022interactive} or features, incorporating edges from the mesh as growth paths introduces a constrain from topological structure, thereby making the growth process more consistent with the geometric structure and avoiding including vertices that are not geometrically related with seed vertices but share similar features with them, making the extraction of object be accurate. 
% A visualization is shown in Fig. ~\ref{fig: grow_vis}. 
We present more analysis on the region-growing algorithm in the supplementary material. 


\begin{comment}
In order to achieve this, we propose the neural surface region growing algorithm which utilizes distilled promptable features in both 2D and 3D spaces. 
The algorithm enables seed vertices growing on the surfaces of foreground mesh based on user instructions, ultimately extracting the surfaces belonging to the target object.
A visualization of neural surface region growing process is shown in Figure ~\ref{fig: grow_vis}.

% An illustration of pipeline of the algorithm
As illustrated in Algorithm.~\ref{surface_growing_alg}, seed vertices and growth boundaries are initially defined based on 2D guidance.
Based on features associated with each vertex, starting from seed vertices, the growth is propagated along the mesh surface, ultimately enabling the extraction of the specified object's surface.
% Given the whole point set $\mathbb P$ derived from the holistic foreground mesh, seed point set $\mathbb S$, boundary point set $\mathbb B$, neighbor set $\Re$ for each point, feature function $\mathcal F$ for each point, a criteria threshold parameter for growing $\tau$, an attenuation parameter $\theta$ and a tolerance $\epsilon$, 
More details about neural surface region growing can be found in Algorithm~\ref{surface_growing_alg}.

% Discuss why we do not use 3D coordinates but edge instead
The geometry relationship between vertices is inherently implied in the definition of the mesh ~\cite{levin1976parametric}.
% From my opinion, the analysis for this part is obvious and no exp is needed
Compared to the growth algorithm that purely refers to spatial location ~\cite{goel2022interactive}, incorporating edges from the mesh as growth paths introduces topological structure, thereby making the growth process more consistent with geometric relationships.
\end{comment}

% Key points I want to address is the following:
% (1.) 2D constraint -> 3D boundary, This propagation works because (or, say why 2D constraint can be appied to 3D as a criteria)
%  - the promptable feature is aligned in multi-view consistent way
% (2.) Basic layout separation improves the robustness of surface growing on 2 aspects:
%  - Despite accurate geometry, 2D-3D matching of contour pixels may bring noisy points from textureless background points, which harms the extraction. Distinguishing between foreground and background allows the surface growing algorithm to operate effectively in low noise environments, enhancing the accuracy of the results and strengthening the algorithm's robustness.

\begin{comment}
\noindent\textbf{Analysis} The key to the success of the neural surface region growing algorithm lies in propagating the 2D guidance into the 3D space. 
The precise mesh extraction is mainly attributed to the following reasons: 
(1)  The distilled 3D features are view consistent and instance-aware. As shown in Figure ~\ref{fig: tsne}, for the features of the same object under different viewpoints, the inter-class distance of the distilled feature pairs is significantly smaller than that of the feature pairs derived from the teacher model ~\cite{kirillov2023segment}.
Thus, with the distilled feature used in both 2D and 3D space, 2D seed pixels and boundary pixels can be reliable references for 3D seed vertices and boundary vertices.
(2) Conducting this process on foreground mesh $\mathcal{M}_F$ allows the algorithm to operate effectively in low-noise environments, enhancing the accuracy of the results and strengthening the robustness.
To be more specific, despite accurate geometry, pixel-vertex matching of contour pixels may bring noisy points from texture-less background, which harms the extraction.
With pure fore-ground mesh for growing, the absence of surfaces originating from the background minimizes interference during the extraction process.
Therefore, these factors collectively enable our method to extract the 3D mesh of a specified object using only a single viewpoint and a few clicks.
(3) The explicit geometry information constrains the growing process of considering the geometric structure and topology of meshes, thus effectively ruling out noise vertices that are not geometrically related. 
(4) The dense object seeds derived from SAM and the boundary constrains, ensuring the quality of propagation. 
\end{comment}

% (3.) Extract thing with only one click within one viewpoint

\begin{figure}[!t]
\vspace{-5pt}
    \centering
    \begin{algorithm}[H]
    \caption{Mesh-based Region Growing}
    \label{surface_growing_alg}
    \begin{algorithmic}[1]
    % \Procedure{SurfaceGrowingAlgorithm}{$\mathbb P$, $\mathbb S$, $\mathbb B$, $\Re$, $\mathcal F$, $\tau$, $\theta$, $\epsilon$}
    \State \textbf{Input:} $\mathcal{V}$ associated with $f_{v_i}$ for each vertex $v_i$, $\mathcal{S}_o$, $\mathcal{B}_o$, $\mathcal{E}$, a similarity threshold $\tau$, an attenuation parameter $\theta$ and a tolerance $\epsilon$
    \State \textbf{Output:} the vertex set $\mathcal{V}_o$ for the object mesh $\mathcal{M}_o$
    \State Initialize the target vertex set $\mathcal{V}_o \gets \mathcal{S}_o$
    \State Initialize the intermediate target vertex set $\mathcal{V}_o' \gets \mathcal{V}_o$
    \State initialize the candidate seed vertex set $\mathcal{S}_o' \gets \emptyset$
    \While{$\mathcal{S}_o \neq \emptyset$}
        \For{each vertex $s$ in $\mathcal{S}_o$}
            \State Find all the neighbors of $s$ with $\mathcal{E}$, as $\mathcal{N}$
            \For{each vertex $n$ in $\mathcal{N}$}
                \State  $\text{sim}(f_s, f_n) \gets \frac{{f_s \cdot f_n}}{{\left\lVert f_s \right\rVert \left\lVert f_n \right\rVert}}$
                \If{$\text{sim}(f_s, f_n) > \tau$} 
                    \State add $n$ to $\mathcal{V}_o'$, add $n$ to $\mathcal{S}_o$
                \Else
                    \State add $s$ to $\mathcal{S}_o'$
                \EndIf
            \EndFor
        \EndFor
        \If{ $\frac{\lvert \mathbb \mathcal{V}_o' \cap \mathcal{B}_o \rvert}{\lvert \mathbb \mathcal{B}_o \rvert} > \epsilon$}
            \State return $\mathcal{V}_o$
        \Else
            \State $\mathcal{V}_o \gets \mathcal{V}_o'$, $\mathcal{S}_o \gets \mathcal{S}_o'$, $\mathcal{S}_o' \gets \emptyset$
        \EndIf
        \State $\tau \gets \tau- \theta$
    \EndWhile
    % \EndProcedure
    \end{algorithmic}
    \end{algorithm}
    \label{fig:enter-label}
    \vspace{-20pt}
\end{figure}

% \begin{figure}[!t]
%     \centering
%     \begin{algorithm}[H]
%     \caption{Mesh-based Region Growing}
%     \label{surface_growing_alg}
%     \begin{algorithmic}[1]
%     % \Procedure{SurfaceGrowingAlgorithm}{$\mathbb P$, $\mathbb S$, $\mathbb B$, $\Re$, $\mathcal F$, $\tau$, $\theta$, $\epsilon$}
%     \State \textbf{Input:} the whole point set $\mathbb P$, seed point set $\mathbb S$, boundary point set $\mathbb B$, neighbor set $\Re$ for each point, feature function $\mathcal F$ for each point, a criteria threshold parameter for growing $\tau$, an attenuation parameter $\theta$ and a tolerance $\epsilon$
%     \State \textbf{Output:} the target set $\mathbb T$
%     \State Initialize the target set $\mathbb T \gets \mathbb S$
%     \State Initialize the intermediate target set $\mathbb T' \gets \mathbb T$
%     \State initialize the intermediate candidate set $\mathbb I \gets \emptyset$
%     \While{$\mathbb S \neq \emptyset$}
%         \State $\tau' \gets \tau - \theta$
%         \For{each point $s$ in $\mathbb S$}
%             \State Find all the neighbors of $s$ given $\mathbb P$, $\mathbb A \gets \Re(s)$
%             \For{each point $a$ in $\mathbb A$}
%                 \State  $similarity \gets \frac{{\mathcal F(a) \cdot \mathcal F(s)}}{{\left\lVert \mathcal F(a) \right\rVert \left\lVert \mathcal F(s) \right\rVert}}$
%                 \If{$similarity > \tau'$} 
%                     \State add $a$ to $\mathbb T$, add $a$ to $\mathbb S$
%                 \Else
%                     \State add $s$ to $\mathbb I$
%                 \EndIf
%             \EndFor
%         \EndFor
%         \If{ $\frac{\lvert \mathbb T \cap \mathbb B \rvert}{\lvert \mathbb B \rvert} > \epsilon$}
%             \State return $\mathbb T'$
%         \Else
%             \State $\mathbb T' \gets \mathbb T$, $\mathbb S \gets \mathbb I$, $\mathbb I \gets \emptyset$
%         \EndIf
%         \State $\tau \gets \tau'$
%     \EndWhile
%     % \EndProcedure
%     \end{algorithmic}
%     \end{algorithm}
%     \label{fig:enter-label}
% \end{figure}



% \section{Applications}
% 1. show examples for applications 









==> sec/4_experiments.tex <==
\section{Experiments}
\label{sec:exp}
\begin{figure*}
% \stepcounter{figure}
  \centering
    % \centering
        \includegraphics[width=0.98\linewidth]{./figure/final_map.pdf}
        \vspace{-5pt}
    \caption{\textbf{Visualized assessments on Replica and ScanNet dataset.} We present the reconstruction results for the background, foreground and decomposed objects. To clearly visualize the decomposed objects, we use different color for the different instances.
    }
    \label{fig: final_results} 
    \vspace{-15pt}
\end{figure*}
\subsection{Experiment Setup}
\paragraph{Implementation Details.} 
Our method is implemented using Pytorch and uses the Adam optimizer with a learning rate of $5e-4$ for the tiny MLP part ( 2 layers with 256 channels for the geometry, appearance, and feature prediction, 1 layer with 128 nodes for the semantic prediction )
% For the geometry MLP, semantic MLP and Feature MLP, we only use two linear layers with 256 nodes.
% As for Semantic MLP, we use a single linear layer with 128 nodes. \xjqi{modify}
In the reconstruction strategy, we minimize the loss
\begin{equation}
\begin{aligned}
    \mathcal{L} = &\mathcal{L}_\text{rgb} +\mathcal{L}_\text{geo} +  \lambda_1\mathcal{L}_{O} + \lambda_2\mathcal{L}_\text{reg} + \\
    &\lambda_3\mathcal{L}_\text{man} +  \lambda_4\mathcal{L}_\text{floor} + \lambda_5\mathcal{L}_\text{sem} + \lambda_6\mathcal{L}_f,\;
\end{aligned}
\end{equation}
to optimize our implicit neural surface, where we set $ \lambda_1, \lambda_2, \lambda_3, \lambda_4, \lambda_5, \lambda_6 $ as $0.1, 0.1, 0.01, 0.01, 0.5, 0.1$, respectively.
More details can be found in the supplementary.
\paragraph{Dataset and Metrics}
Our experiments are mainly conducted on the \textbf{Replica}~\cite{replica19arxiv} dataset, which is a synthetic dataset with each providing accurate geometry, HDR textures and 3D instance annotations.
We follow the selection of ObjSDF++~\cite{wu2023objectsdf++} to evaluate the effectiveness of our method.
We report both instance-level and holistic reconstruction results on this dataset.
The reconstruction results are mainly evaluated by Chamfer-$L_1$ and F-Score. 
To further demonstrate the robustness of our method, we also use the \textbf{ScanNet}~\cite{dai2017scannet} as the real-world dataset which provides 1513 scenes.
Due to its lack the object object-level ground truth, we show the visualized assessment in the main paper.
More details and results can be seen in the supplementary.

\paragraph{Compared Methods.}
The compared methods are mainly divided into two categories. 
The first one is the object compositional reconstruction method that uses multiple fields to represent each object with the supervision from ground truth instance masks, like ObjSDF++~\cite{wu2023objectsdf++}. 
We compare the instance level and holistic scene reconstruction quality with them. 
The second category is the volume density based methods that decompose each scene with generalized features, like ISRF~\cite{goel2022interactive}, DFF~\cite{kobayashi2022decomposing}.
Since this type of method does not introduce geometric constraints, we mainly compare the way of decomposition.

\subsection{Results}
\vspace{-10pt}
\begin{table}[h]
    \centering \scalebox{0.75}{
    \renewcommand\arraystretch{1.3}
    \begin{tabular}{c|cc|cc}
        \bottomrule[0.9pt] & \multicolumn{2}{c|}{Scene Reconstruction} & \multicolumn{2}{c}{Decomposed Reconstruction} \\
        \textbf{Method} & Chamfer-$\mathcal{L}_1$ $\downarrow$  & F-score $\uparrow$ & Chamfer-$\mathcal{L}_1$ $\downarrow$  & F-score $\uparrow$ \\ 
        \hline
        ObjSDF++ & 3.58 & 85.69 & 3.84 $\pm$ 0.02 & 79.49 $\pm$ 0.08\\
        \hline
        \emph{Ours} & \textbf{3.53} & \textbf{85.82} & \textbf{3.58} $\pm$ 0.01 & \textbf{81.70} $\pm$ 0.08\\
        \toprule[0.9pt]
    \end{tabular}
        }
    \vspace{-10pt}
    \caption{Quantitative assessments from Replica dataset on scene and decomposed reconstruction.}
    \label{tab: replica_results}
\vspace{-30pt}
\end{table}
\paragraph{Scene reconstruction and object decomposition on the Replica dataset.}
To evaluate the decomposed reconstruction accuracy of \textit{Total-Decom}, we conduct experiments on the Replica dataset as {it provides ground-truth objects' meshes for evaluation}. 
We mainly compared our approach with the ObjSDF++, the state-of-the-art method that decomposes the scene structure with pseudo geometry priors as far as we know.
Because the number of decomposed objects from ObjSDF++ is limited (around 25 objects per scene), we only evaluate the foreground objects that ObjSDF++ can extract for a fair comparison. In reality, our approach can generally yield a more complete decomposition of the scene with more objects.
The results are shown in  Table~\ref{tab: replica_results}.
%As shown in the third row of Fig.~\ref{fig: final_results}, the ObjSDF++ can decompose the scene but requires the ground-truth instance segmentation masks.
Although our approach doesn't rely on ground-truth instance masks for decomposition, our method still surpasses ObjSDF++ in both scene and decomposed object reconstruction results.
It is worth noting that our approach only requires 1.41 clicks on average per object, while ObjSDF++ requires dense human instance annotations on multi-view images.  
%One reason is that multiple SDF fields of different objects will exceed the capability of one implicit representative network, which decreases the reconstructed details and accuracy.
Our reconstructed results also outperform ObjSDF++ qualitatively. 
As shown in Fig.~\ref{fig: final_results}, ObjSDF++ tends to inaccurately reconstruct the vase (\textit{Room\_0}) and trash bin (\textit{Office\_4}) within the background field or may fail to recover the structure of the chair (\textit{Office\_4}). 
%In contrast, our method utilizes only two SDF fields to model the entire scene, which alleviates the burden of the MLP representation, leading to better scene reconstruction results.
 With an elaborately mesh-based region-growing method facilitated by SAM, our method can deliver decomposed results of higher qualities.

\begin{table}[b]
  \centering
    \vspace{-10pt}
    \begin{adjustbox}{width=\linewidth}
  % \scriptsize
    \scriptsize
    \begin{tabularx}{\linewidth}{c|cccc}
        \bottomrule[1pt]
         % \multirow{3}{*}{Method} & \multirow{3}{*}{Accurate Geometry} &  \multirow{3}{*}{Multi-grained Decomposition} &  \multirow{3}{*}{} &  \multirow{3}{*}{}\\ 
         % \\
         \makecell{Method} & \makecell{Geometry} & \makecell{Multi-grained} & \makecell{Scene-level} & \makecell{Single-View \\ Interaction} \\
        \hline
        LSeg + DFF ~\cite{kobayashi2022decomposing} & \hspace{0pt} \ding{55} & \hspace{0pt} \ding{55}  & \hspace{0pt} \ding{55} & \hspace{0pt} \ding{55}   \\
        \makecell{DINO +\\ DFF/N3F~\cite{tschernezki2022neural}} & \hspace{0pt} \ding{55} & \hspace{0pt} \checkmark  & \hspace{0pt} \ding{55} & \hspace{0pt} \ding{55}  \\
        ISRF ~\cite{goel2022interactive} & \hspace{0pt} \ding{55} & \hspace{0pt} \checkmark  & \hspace{0pt} \ding{55} & \hspace{0pt} \ding{55}  \\
        SAMNeRF ~\cite{cen2023segment} & \hspace{0pt} \ding{55} & \hspace{0pt} \checkmark  & \hspace{0pt} \ding{55} & \hspace{0pt} \ding{55}  \\
        \makecell{Panoptic \\ Lifting}~\cite{siddiqui2022panoptic}  & \hspace{0pt} \ding{55} & \hspace{0pt} \ding{55}  & \hspace{0pt} \checkmark & \hspace{0pt} \ding{55} \\
        AssetField ~\cite{xiangli2023assetfield} & \hspace{0pt} \ding{55} & \hspace{0pt} \ding{55}  & \hspace{0pt} \checkmark & \hspace{0pt} \ding{55} \\
        vMAP ~\cite{kong2023vmap} & \hspace{0pt} \checkmark  & \hspace{0pt} \ding{55}  & \hspace{0pt} \checkmark & \hspace{0pt} \ding{55} \\
        ObjSDF++ ~\cite{wu2023objectsdf++} & \hspace{0pt} \checkmark  & \hspace{0pt} \ding{55}  & \hspace{0pt} \checkmark & \hspace{0pt} \ding{55} \\
        \emph{Ours} &  \hspace{0pt} \checkmark  & \hspace{0pt} \checkmark  &  \hspace{0pt} \checkmark & \hspace{0pt} \checkmark\\ \toprule[1pt]
    \end{tabularx}
  % }
      \end{adjustbox}
    \vspace{-10pt}
    \caption{Comparison of decomposition capabilities between different methods.}
%     \label{tab:ablation}
% \vspace{-0.2cm}
% \end{table}
  \label{tab: ability_com}
  % \vspace{-25pt}
\end{table}

\paragraph{Background reconstruction.}
We demonstrate the quality of background reconstruction in Fig.~\ref{fig: manhattan} and  Fig.~\ref{fig: final_results}. 
Our approach consistently delivers high-quality clean background reconstructions and reconstructs occluded areas. 
%In Fig.~\ref{fig: manhattan}, we have already shown the effect of our newly proposed constraint to the background field on the \textit{room\_1} in the Replica dataset.
%Moreover, we also show additional reconstructed results in the Fig.~\ref{fig: final_results}.
%Clearly, our method demonstrates sufficient robustness across different scenes including synthetic and real dataset, allowing use to perform cross-scene editing without any constraints.

\paragraph{Comparison of Decomposition Capabilities}
We compare the decomposition capabilities of our model with existing methods in NeRF and 3D reconstruction in terms of whether they can support geometric decomposition, multi-grained decomposition, scene-level decomposition, and interactive selection. Tab.~\ref{tab: ability_com} presents the comparison results, indicating that our method is the sole approach encompassing all capabilities. Additional results and applications exploiting these capabilities can be found in the supplementary material.

%We compare the decomposition ability of our model with existing methods in NeRF and 3D reconstruction. 
%Generally, we attribute the decomposed capability to the following aspects: geometric decomposition, multi-grained decomposition, scene-level decomposition, and interactive selection.
%The comparison results are listed in Tab.~\ref{tab: ability_com}, which shows that our method is the only approach possessing all capabilities. We show more results and applications leveraging these capabilities in the supplementary file. 

% \paragraph{Scene editing}
% Because of the 

% \paragraph{Room re-decoration with generative model}
% \paragraph{Reconstruction on the self-captured scene}
% \subsection{Geometry-driven animating}

==> sec/5_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We presented \textit{Total-Decom}, a novel framework for reconstructing a 3D surface and decomposing it into individual objects and backgrounds, significantly reducing the reliance on object annotations. Our approach centers on integrating SAM with hybrid implicit-explicit surface representations and a mesh-based region-growing algorithm. SAM provides object-aware features and facilitates the acquisition of more accurate object seeds for region growth. Simultaneously, the region-growing algorithm effectively combines geometric topology from explicit mesh and object-aware features from SAM to accurately decompose desired objects with minimal human annotations. Qualitative and quantitative evaluations indicate that our method can yield not only precise geometry but also extract as many objects as possible. We hope our proposed method will facilitate the development of environment simulators in the future. 
% \xjqi{We include limitation analysis in the supplementary file.} 

%We have presented  \textit{Total-Decom}, a novel framework to reconstruct a 3D surface and decompose it into individual objects and backgrounds while significantly reducing the need for object annotations. 
%The core of our approach is combining SAM with hybrid implicit-explicit surface representations and a mesh-based region-growing algorithm. SAM provides object-aware features and facilitates obtaining more accurate object seeds for region growth. Meanwhile, the region-growing algorithm effectively combines the geometric topology from explicit mesh and object-aware features from SAM to accurately decompose desired objects while requiring minimal human annotations. 
%Qualitative and quantitative assessments demonstrate our method can not only yield accurate geometry but also extract objects as many as possible.
%We envision our proposed method will be the core component to support further endeavors in building environment simulators. 
\begin{comment}
   We leverage easily obtained 2D segmentation masks to separately reconstruct the foreground and background meshes, on which we also distilled the learned SAM features on the vertices.
At any poses, we use the rendered feature and user clicked prompts into the SAM decoder to masked interested 2D regions.
Thanks to the tailored {mesh-based region-growing method}, we can directly extract the 3D structure of any desired objects. 
\end{comment}
%By incorporating  SAM features into the reconstructed meshes vertices, \textit{Total-Decom} can decompose the scene into background, foreground, and objects levels.
%Qualitative and quantitative assessments demonstrate our method can not only decompose the accurate geometry but also extract objects as any as possible.
%We envision our proposed method will be the core components to build the virtual simulator.



==> sec_bak/0_abstract.tex <==
\begin{abstract}
% Briefly introduce the research question/focus to make the task clear
%
Neural implicit 3D scene reconstruction in a decomposed form, which represents a scene using object-level compositional components and background, is a challenging yet crucial research problem with significant implications for numerous real-world applications, such as simulation and scene editing.
% Point out the weakness of previous work
% Main weakness 1: Uncontrolled Scalability
%
Existing methods utilize separate neural networks to represent individual objects, leading to scalability issues, as the network size must increase with the number of object instances. 
% Main weakness 2: acquisition of labels
%
Additionally, they rely on multi-view consistent instance-level dense labels, which are difficult to acquire in real-world scenes. %, further limiting their downstream applications.
% Motivation and a brief introduction to our solution
%
To address these challenges, this paper introduces a novel method that can reconstruct the holistic scene and decompose it in a complete manner. %, while ensuring the plausibility of the occluded surfaces in the background of the scene.
% Overview of the pipeline
%
We first represent the entire scene in a bilayer form, leveraging depth and semantic information to ensure that objects in the scene can be distinguished from the background, e.g., walls or floors, which belong to a different layer. %, and optimize the surfaces belonging to each layer separately. 
Scenic priors, particularly plane constraints, are employed to facilitate high-quality reconstruction in occluded regions.
We further integrate 2D general features from the segment anything model, allowing users to interactively select any object in the scene.
Our method further propagates the 2D user-specified 'objectness' through neural implicit representation to the 3D space, using a novel surface growing algorithm to extract the corresponding 3D object without additional interaction. 
% Illustrate the result and address the two weakness once again
Extensive experimental results validate the effectiveness of our approach, showcasing its ability to generate high-fidelity outputs for complex holistic scenes and handle a large number of objects without need of instance-level labels.
\end{abstract}

% Previous version & Comments
%\xjqi{please modify this part}Decomposed de-occluded \xjqi{no de-occlued??} neural implicit 3D scene reconstruction, which represents a scene as a collection of de-occluded 3D objects and background, is a challenging yet crucial research problem with numerous real-world applications, such as simulation and scene editing. 
% Existing methods utilize separate neural networks to represent individual objects, leading to scalability issues, as the network size must increase with the number of object instances. 
% Furthermore, these methods often neglect the surface quality of invisible regions, resulting in unsatisfactory reconstruction of occluded areas \xjqi{no this part}.
% To address these challenges, this paper introduces a new method for reconstructing and decomposing any 3D instances, including their invisible surfaces. 
% We first decompose the scene into multiple layers along the vertical direction, leveraging depth and semantic information to ensure objects and backgrounds are not occluded within a single layer, and reconstruct them hierarchically. 
% Scenic priors, particularly plane constraints, are employed to facilitate high-quality reconstruction in occluded regions.
% Subsequently, given the reconstructed decomposed de-occluded 3D scene, we incorporate an interactive interface that leverages 2D promptable segmentation obtained from the Segment Anything Model and a novel surface-growing algorithm to segment any desirable 3D object according to user instructions. 
% Extensive experimental results validate the effectiveness of our approach, showcasing its ability to generate high-fidelity outputs for complex holistic scenes and handle a large number of instance-level objects.

==> sec_bak/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
\xjqi{(1) Scene reconstruction from sparse multi-view images has been a fundamental problem in computer vision and graphics \xjqi{add citations}. (2) Recently, neural radiance fields xxxx with xxx xxx representations have been proposed for this task. (3) Although advancements have been achieved, editing/manipulating a 3D geometry of a reconstructed scene, such as xxx, controlled by users remains a challenging problem due to [the composed nature of xxx]. (4) Thus, we study decomposed 3D reconstruction which is an under-explored yet important problem for many real-world applications such as xxx xxx.   }

Indoor scene reconstruction from sparse multi-view images has been a fundamental problem in computer vision and graphics~\cite{yu2022monosdf, guo2022neural, sun2021neuralrecon}.

Scene decomposition has long been a subject of inquiry in computer vision and computer graphics. 
It aims to enhance interaction with the desired 3D structure and visual content, creating a more immersive virtual world and enabling various applications in embodied simulation. 
Recently, neural volumetric representations like neural radiance field (NeRF)~\cite{mildenhall2021nerf} have emerged, acting as a bridge between rendering, perception, and reconstruction. 
This breakthrough allows the integration of perceptual findings to decompose the outcomes of reconstruction and rendering processes.
These representations utilize volume density, occupancy\cite{oechsle2021unisurf}, signed distance functions (SDF)\cite{wang2021neus, yariv2021volume}, or hybrid variations\cite{Lyu_2023_ICCV}, along with multilayer perceptrons (MLPs) and hash grids~\cite{mueller2022instant, yu2022monosdf}, to map input positions to volumetric functions, view-dependent emitted radiance, and semantic information~\cite{zhi2021place}. 
Neural rendering techniques are then applied to synthesize these properties along a single ray and obtain the pixel value.


\xjqi{1. There are some early attempts on decomposed 3D reconstruction which, however, [mlpsxxx] relies on human-annotated instance-level masks for decomposition \xjqi{objnerf and objectnerf++??} \xjqi{caanot control granurity}. 2. Besides, distilling generalized features from pre-trained image backbones such as xxx xxx have been used for developing decomposed neural radiance field, focusing one neural rendering qualities.....Applying xx to reconstruction remain xxx [add drawbacks]. }

Incorporating perceptual capabilities, there are two mainstream approaches to decompose a room-level scene using neural implicit representation:
(1) Object Compositional Reconstruction:
These approaches use ground truth instance segmentation masks or bounding boxes to partition the holistic scene into multiple implicit fields. 
Subsequently, compositional functions are employed to amalgamate these fields into a unified whole. 
While they achieve accurate geometry for any instance, they heavily rely on precise labeling, limiting the level and quantity of decomposition.
(2) Decomposed Scenes with Generalized Features:
These methods aim to decompose scenes with generalized features, distilling them into volumetric representations. 
Features include L-Seg~\cite{li2022language}, CLIP~\cite{radford2021learning}, and DINO~\cite{caron2021emerging}. 
An attention-based selection technique identifies specific visual regions after traversing the 3D space. 
However, these methods emphasize novel view synthesis, potentially neglecting geometric accuracy.
Directly applying these strategies to the implicit SDF field~(Fig.~\ref{fig: distill features}), results in decomposition outputs that may lack well-defined contours, and may not enable the extraction of independent instance segmentation results, thus significantly affecting downstream applications, such as animations.

\xjqi{1. In this paper, we present xxx tailored to decomposed 3D reconstruction with minimal human interactions which decomposes the geometry of a 3D scene into xxx and allows xxx editing.  2. Our method seamlessly incorporates an interactive segmentation model -- SAM -- into a neural implicit reconstruction model to allow users to control xxx for reconstructing and modifying the desirable regions \xjqi{objects or parts} with one click??.  }

Therefore, this paper introduces the Total-Decom framework to reduce dependence on 2D instance segmentation masks while obtaining a comprehensive representation of instance-level geometry. 
Using easier-obtained foreground and background segmentation masks, we achieve a preliminary scene division. In the foreground field, promptable generalized features, like the Segment Anything Model feature~\cite{kirillov2023segment}, enable meticulous segmentation. 
This approach improves reconstruction quality for scenes and objects and achieves complete decomposition of indoor scenes at an instance level.

\xjqi{Specifially, We first train a xxx augmented with feature rendering and background-foreground partition . Then, for xxx, we distill the features into meshes for interactive selection, rendering and xx in real time with is combined with a segmentation decoder for xxx. For accurately xxx, we develop a xxxx . Finally, xxx }

To accommodate the traits of promptable features and enable the direct selection of desired meshes from any viewpoint, we devised a mesh-based surface growing algorithm (Section~\ref{subsec: surface}). 
This algorithm utilizes generalized features distilled onto mesh vertices, enabling us to acquire the precise geometric structure of any object from a single frame. 
Notably, this approach eliminates the need for iterative rendering to obtain the 3D structure of the object, a requirement present in prior methods.
Furthermore, to enhance the interactive experience, we have made modifications to the Gaussian Splatting~\cite{kerbl3Dgaussians} technique. 
This adaptation allows us to render images on fixed mesh vertices, opening the door to real-time interactivity with the reconstructed mesh, encompassing both its geometry and rendering aspects.

Overall, our main contributions are as follows: \xjqi{looks fine, we can revise it later}
\begin{itemize}
    \item Introduction of an innovative decomposed reconstruction pipeline, achieving comprehensive 3D scene decomposition. 
    This relies on easily obtained foreground and background segmentation masks, coupled with generalized promptable features.
    \item Proposal of a neural mesh-friendly surface-growing algorithm, facilitating the selection of objects of interest from any viewpoint.
    \item Design of an intuitive GUI, enabling interactive object editing directly from the neural radiance field.
    \item Comprehensive evaluation of our method on diverse datasets, showcasing its ability to decompose more objects in a user-friendly manner. Additionally, demonstration of significant potential for various downstream tasks, including animation and scene editing.
\end{itemize}

% Scene decomposition has long been a subject of investigation in the fields of computer vision and computer graphics. 
% It will enhance the interaction with the desired 3D structure and visual content in order to create a more immersive virtual world and enable various applications in embodied simulation.
% Recently, neural volumetric representations such as neural radiance field (NeRF)~\cite{mildenhall2021nerf} have emerged as a compelling bridge to connect the rendering with perception and reconstruction.
% This breakthrough facilitates the integration of perceptual findings to decompose the outcomes of both reconstruction and rendering processes.
% The majority of these approaches utilize representations in the form of volume density, occupancy\cite{oechsle2021unisurf}, signed distance functions (SDF)~\cite{wang2021neus, yariv2021volume}, or hybrid variations thereof~\cite{Lyu_2023_ICCV}. 
% These representations are employed in conjunction with multilayer perceptrons (MLPs) and hash grids~\cite{mueller2022instant, yu2022monosdf} to map the input positions to the volumetric function, view-dependent emitted radiance, and semantic information~\cite{zhi2021place}.
% Subsequently, neural rendering techniques are employed to synthesize the aforementioned properties along a single ray and obtain the pixel value.

% Incorporating perceptual capabilities, neural volumetric representations have commonly delineated scenes into two distinct categories:
% (1) Object Compositional Reconstruction~\cite{wu2022object, wu2023objectsdf++, li2023rico, kong2023vmap}:
% These approaches utilize ground truth instance segmentation masks or bounding boxes to partition the holistic scene into multiple implicit fields. Subsequently, compositional functions are employed to amalgamate these fields into a unified whole. 
% Although they can obtain accurate geometry results for any instance, these techniques heavily rely on precise and detailed labeling, thereby constraining the level and quantity of decomposition.
% (2) Decomposed Scenes with Generalized Features~\cite{kobayashi2022decomposing, goel2022interactive, tschernezki2022neural, wang2023autorecon, lerf2023}:
% These methods aim to decompose the scenes with generalized features. They always distill features into volumetric representations, such as L-Seg~\cite{li2022language} features, CLIP features~\cite{radford2021learning}, and DINO~\cite{caron2021emerging} features, et al. 
% Subsequently, an attention-based selection technique is employed to identify specific visual regions after traversing the entirety of the 3D space.
% However, these approaches predominantly emphasize the quality of novel view synthesis while potentially overlooking the importance of geometric accuracy. 
% Directly applying these strategies to the implicit SDF field~(Fig.~\ref{fig: distill features}), results in decomposition outputs that may lack well-defined contours, and may not enable the extraction of independent instance segmentation results, thus significantly affecting downstream applications, such as animations.

% Therefore, this paper presents the Total-Decom framework, which is designed to reduce dependence on 2D instance segmentation masks and concurrently acquire a comprehensive and accurate representation of instance-level geometry.
% Inspired by the strengths of two leading decomposition approaches, we employ readily attainable foreground and background segmentation masks (encompassing elements such as walls, floors, and ceilings) to create a preliminary division of the scene into two distinct fields. 
% Within the foreground field, we distilled promptable generalized features, such as the Segment Anything Model feature~\cite{kirillov2023segment}, to execute meticulous and fine-grained segmentation of the entire scene.
% With this approach, we can not only enhance the quality of reconstruction for both scenes and objects but also achieve a complete decomposition of indoor scenes at an instance level.

% To accommodate the traits of promptable features and enable the direct selection of desired meshes from any viewpoint, we devised a mesh-based surface growing algorithm (Section~\ref{subsec: surface}). 
% This algorithm utilizes generalized features distilled onto mesh vertices, enabling us to acquire the precise geometric structure of any object from a single frame. 
% Notably, this approach eliminates the need for iterative rendering to obtain the 3D structure of the object, a requirement present in prior methods.
% Furthermore, to enhance the interactive experience, we have made modifications to the Gaussian Splatting~\cite{kerbl3Dgaussians} technique. 
% This adaptation allows us to render images on fixed mesh vertices, opening the door to real-time interactivity with the reconstructed mesh, encompassing both its geometry and rendering aspects.

% Overall, our main contributions are as follows.
% \begin{itemize}
%     \item We propose a new decomposed reconstruction pipeline to totally decompose a 3D scene relying on the easier obtained foreground and background segmentation masks and generalized prompotable feature.
%     \item We propose a neural mesh-friendly surface-growing algorithm that can help us to select the interested objects in any view.
%     \item We design an easy-to-use GUI to interactively edit any objects from neural radiance field. 
%     \item We evaluate our method on different datasets and demonstrate that our method can decompose more objects in a more user-friendly manner, and also show great potential with many downstream tasks like animation and scene editing.
% \end{itemize}

% Previous version & comments
% \xjqi{P1: what's the problem, why is it important. [you may emphasis interactive if needed]
% We explore the problem of decomposed 3D reconstruction and rendering [not sure whether we emphasize rendering or not??], aiming to recover the geometry of xxx and xx, from a few posed images [refer to teaser images]. This is an important research problem that enables many applications in embodied simulation, scene editing, ... }

% \xjqi{P2. 1. a general summary of existing methods for decomposition. Better categorize them into multiple streams. (stream 1: object nerf, object nerf++. [not sure whether we mention a) label space distillation?? panoptic lifting and so on. b) feature space decompostion (DINO feature) c) DM-NeRF] Summarize each stream of work and their advantages and limitations. [maybe we can focus on approaches that focus on evaluating reconstruction capability and leave other methods into the related work] 3. Motivate your solution  }


% \xjqi{P3. Your solution and pipeline 1. the first sentence to summarize your approach. 2 several sentences to describe key components of your methods and link them as a coherent story. We first put forward a feature xxxx. Then, to xxx, we xxxx. [write as we discussed]  3. analyze and summary echo why your problem address aforementioned issues (echo P2.)}

==> sec_bak/2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}
%\xjqi{more citations should be discussed such as DM-NeRF especially their papers mentioned decomposed reconstruction}
\paragraph{Object Compositional Reconstruction}
In order to better reconstruct the geometry of internal objects in complex indoor scenes, many research efforts have been devoted to exploring better representations at the object-compositional scene level. ObjSDF \cite{wu2022object} proposes an object-compositional scene representation to assist in geometry optimization in highly composite scenes and better object-level extraction with the help of multi-view consistent instance label. vMAP \cite{kong2023vmap} builds an object-level scene model from a real-time RGB-D input stream to solve object-compositional SLAM. ObjSDF++ \cite{wu2023objectsdf++} builds upon the object-compositional scene representation and further mitigates object collisions in complex scenes through an object distinction regularization term. Additionally, it introduces a new occlusion-aware object opacity rendering scheme to reduce the negative impact of occlusion on scene reconstruction. However, these methods rely heavily on accurate multi-view consistent instance-level labels, resulting in limitations in their down-stream applications on in-the-wild data from the real world.

\paragraph{Decompositional Neural Rendering} In the field of decompositional neural rendering, many research efforts investigate the distillation of generalized features~\cite{lerf2023, goel2022interactive, kobayashi2022decomposing} or segmentation predictions~\cite{siddiqui2022panoptic, bing2022dm} from large-scale pre-trained image backbones, such as DINO~\cite{caron2021emerging}, CLIP features~\cite{radford2021learning} and panoptic segmentation~\cite{cheng2022masked}, to neural fields. 
These approaches leverage feature similarities or predicted instance/semantic codes for grouping and implicitly decomposing a scene, requiring no additional human annotation efforts and offering greater scalability for large-scale scenes.
However, when directly applied to the reconstruction task, these strategies often produce decomposed outputs that are incomplete and exhibit poorly defined contours (see Fig. \xjqi{xxx}) due to ill-defined object boundaries \xjqi{add citations} or multiview inconsistent and low-quality segmentation predictions  \xjqi{add citation} used during training. 

\paragraph{Decompositional Neural Rendering}
\xjqi{please merge this paragraph with the above one and rewrite the related work}
% Background
The field of Decomposition of neural implicit representation has witnessed significant progress in recent research \cite{kobayashi2022decomposing, tschernezki2022neural,goel2022interactive,jambon2023nerfshop}.
% No feature distillation
NeRFshop \cite{jambon2023nerfshop} utilizes geometric cues to select objects in a scene, but the lack of objectness awareness often leads to the omission of certain parts of the target objects or the inclusion of background information in the selection process. 
% Semantic feature & General feature distillation
Some alternative methods attempt to address this problem from the perspective of semantics. 
Semantic NeRF \cite{zhi2021place} explores incorporating regressing semantic labels into the process of Novel View Synthesis.
Building upon this, Distilled Feature Fields (DFFs) \cite{kobayashi2022decomposing} and Neural Feature Fusion Fields (N3F) \cite{tschernezki2022neural} have emerged as pioneering approaches for distilling \cite{hinton2015distilling} semantic features from pretrained models, such as LSeg \cite{li2022language} and DINO \cite{caron2021emerging}, into NeRF for decomposition. 
ISRF \cite{goel2022interactive} does not rely solely on feature matching, but instead obtains the final results through region growing.
Due to the limitations of these features, as well as the lack of further design in existing methods, users inevitably rely on extensive interactions to obtain an expected selection result, contradicting the initial design intention of labor-saving.
% Promptable feature
Segment Anything Model (SAM) \cite{kirillov2023segment} achieves efficient 2D interactive segmentation capabilities through extensive high-quality annotated supervision. 
It brings forth more possibilities in this field and opened up new avenues for exploration.
% Focus on 3D representaion
Existing research has devoted significant efforts to decomposition in terms of visual rendering, but extracting the constituent parts as fundamental 3D representations, such as mesh, from the scene still remains an underexplored area with limited research.
AutoRecon \cite{wang2023autorecon} enables reconstructing the main objects in a scene in n a decompositional manner, but it is specifically designed for object-centric scenes.
% Conclude about our work
In contrast to existing methods, our work not only avoids the need for extensive manual interaction through a geometry-guided feature approach but also enables the extraction of 3D meshes for the constituent parts of the scene.
\xjqi{mention SAM and NeRF combination works}


% \section{Related Work}
% \label{sec:related_work}
% %\xjqi{more citations should be discussed such as DM-NeRF especially their papers mentioned decomposed reconstruction}
% \paragraph{Object Compositional Reconstruction}
% In order to better reconstruct the geometry of internal objects in complex indoor scenes, many research efforts have been devoted to exploring better representations at the object-compositional scene level. ObjSDF \cite{wu2022object} proposes an object-compositional scene representation to assist in geometry optimization in highly composite scenes and better object-level extraction with the help of multi-view consistent instance label. vMAP \cite{kong2023vmap} builds an object-level scene model from a real-time RGB-D input stream to solve object-compositional SLAM. ObjSDF++ \cite{wu2023objectsdf++} builds upon the object-compositional scene representation and further mitigates object collisions in complex scenes through an object distinction regularization term. Additionally, it introduces a new occlusion-aware object opacity rendering scheme to reduce the negative impact of occlusion on scene reconstruction. However, these methods rely heavily on accurate multi-view consistent instance-level labels, resulting in limitations in their down-stream applications on in-the-wild data from the real world.

% \paragraph{Decompositional Neural Rendering} In the field of decompositional neural rendering, many research efforts investigate the distillation of generalized features~\cite{lerf2023, goel2022interactive, kobayashi2022decomposing} or segmentation predictions~\cite{siddiqui2022panoptic, bing2022dm} from large-scale pre-trained image backbones, such as DINO~\cite{caron2021emerging}, CLIP features~\cite{radford2021learning} and panoptic segmentation~\cite{cheng2022masked}, to neural fields. 
% These approaches leverage feature similarities or predicted instance/semantic codes for grouping and implicitly decomposing a scene, requiring no additional human annotation efforts and offering greater scalability for large-scale scenes.
% However, when directly applied to the reconstruction task, these strategies often produce decomposed outputs that are incomplete and exhibit poorly defined contours (see Fig.~\ref{fig: selected_mesh}) due to ill-defined object boundaries~\cite{goel2022interactive} \xjqi{add citations} or multiview inconsistent and low-quality segmentation predictions~\cite{wang2022dm}  \xjqi{add citation} used during training. 

% \paragraph{Decompositional Neural Rendering}
% \xjqi{please merge this paragraph with the above one and rewrite the related work}
% % Background
% The field of Decomposition of neural implicit representation has witnessed significant progress in recent research \cite{kobayashi2022decomposing, tschernezki2022neural,goel2022interactive,jambon2023nerfshop}.
% % No feature distillation
% NeRFshop \cite{jambon2023nerfshop} utilizes geometric cues to select objects in a scene, but the lack of objectness awareness often leads to the omission of certain parts of the target objects or the inclusion of background information in the selection process. 
% % Semantic feature & General feature distillation
% Some alternative methods attempt to address this problem from the perspective of semantics. 
% Semantic NeRF \cite{zhi2021place} explores incorporating regressing semantic labels into the process of Novel View Synthesis.
% Building upon this, Distilled Feature Fields (DFFs) \cite{kobayashi2022decomposing} and Neural Feature Fusion Fields (N3F) \cite{tschernezki2022neural} have emerged as pioneering approaches for distilling \cite{hinton2015distilling} semantic features from pretrained models, such as LSeg \cite{li2022language} and DINO \cite{caron2021emerging}, into NeRF for decomposition. 
% ISRF \cite{goel2022interactive} does not rely solely on feature matching, but instead obtains the final results through region growing.
% Due to the limitations of these features, as well as the lack of further design in existing methods, users inevitably rely on extensive interactions to obtain an expected selection result, contradicting the initial design intention of labor-saving.
% % Promptable feature
% Segment Anything Model (SAM) \cite{kirillov2023segment} achieves efficient 2D interactive segmentation capabilities through extensive high-quality annotated supervision. 
% It brings forth more possibilities in this field and opened up new avenues for exploration.
% % Focus on 3D representaion
% Existing research has devoted significant efforts to decomposition in terms of visual rendering, but extracting the constituent parts as fundamental 3D representations, such as mesh, from the scene still remains an underexplored area with limited research.
% AutoRecon \cite{wang2023autorecon} enables reconstructing the main objects in a scene in n a decompositional manner, but it is specifically designed for object-centric scenes.
% % Conclude about our work
% In contrast to existing methods, our work not only avoids the need for extensive manual interaction through a geometry-guided feature approach but also enables the extraction of 3D meshes for the constituent parts of the scene.
% \xjqi{mention SAM and NeRF combination works}




==> sec_bak/3_method.tex <==
% Our goal is to totally decompose (at any granularity) and edit the reconstructed mesh with the user-friendly interactive method.
% Firstly, we use machine-generated foreground and background segmentation masks to automatically reconstruct an indoor scene into two different fields.
% Applying the object distinct loss and unobserved Manhattan loss, we can get the pure foreground mesh~\ref{fig: fg_mesh} and a completely clean background mesh~\ref{fig: bg_mesh}.
% In the meantime, we distill the generalized features like the segment anything model features on the vertices of the two field meshes.
% Subsequently, we develop a new graphic interactive application that uses the vertices of the holistic reconstructed mesh as the fixed point to fit the 3D Gaussian~\cite{kerbl3Dgaussians} to perform real-time image rendering.
% Incorporating the distillation features and SAM decoder, our newly designed surface-based region-growing algorithm allows us to select any objects or parts at any view with only one click.
% Besides, the Total-Decom pipeline can support many other interesting downstream applications like interacting with objects~\ref{fig: application}, cross-scene editing~\ref{fig: application}, room re-texture~\ref{fig: application} et al.

This section describes the proposed approach for indoor scene front-background separated reconstruction and total decomposition for the scene. 
% % % I prefer to address one of our most important key insights: decompose the scene from both aspects of geometry and semantics again here
To reach total decomposition, geometry and semantics matter both. 
The proposed approach consists of two main stages: front-background separated reconstruction (Section~\ref{sec: separated reconstruction}) and promptable decomposition (Section~\ref{sec:promptable decomposition}).
An overview of our approach is presented in Figure \ref{fig:pipeline}.
%
\subsection{Front-background separated reconstruction}
\label{sec: separated reconstruction}
\subsubsection{Preliminary}
Here, we describe the mathematical preliminary of the implicit neural surface reconstruction methods.
\paragraph{SDF-based scene representation.}
We represent the scene as a signed distance function (SDF) field, which is a continuous function $f$ that calculates the distance between each point and its closest surface.
Following InstantNGP~\cite{mueller2022instant} and VolSDF~\cite{yariv2021volume}, we use hierarchical explicit grids and shallow MLP to represent the function $f$ and convert the SDF value to Laplace density with the following function
\begin{equation}
    \sigma_i(\boldsymbol{p}_i)=\alpha \Psi_\beta\left(-f(\boldsymbol{p}_i)\right) \;,
\end{equation}
where $\alpha, \beta > 0$ are learnable parameters and $\Psi_\beta$ is the cumulative distribution function (CDF) with zero mean and the $\beta$ scale is defined as
\begin{equation}
    \Psi_\beta(d)= \begin{cases}
    \frac{1}{2} \exp \left(\frac{d}{\beta}\right) &, \text { if } s \leq 0 \\ 1-\frac{1}{2} \exp \left(-\frac{d}{\beta}\right) &, \text { if } s>0
    \end{cases} ,
\end{equation}
where $d$ is the signed distance function.

\paragraph{Rendering Formula}
According to the rendering formula~\cite{mildenhall2021nerf, kobayashi2022decomposing, zhi2021place, yu2022monosdf}, we use $T_i^r$ and $\alpha_i$ to represent the transmittance and alpha value of sample points, which can be computed by
\begin{equation}
        T^r_i = \prod_{j=1}^{i-1}(1-\alpha_i), ~
    \alpha_i = 1 - \exp(-\sigma^r_i\delta^r_i) \;,
\end{equation}
where $\delta^r_i$ is the distance between adjacent sample points.
Thus, we can render the color, surface normal, and depth along the ray $r$ by
\begin{equation}
    \label{eq: rendering_formula}
    \hat{C}(r) = \sum_{i=1}^{M}T^r_i\alpha_i\hat{c}^r_i \;,
    \hat{D}(r) = \sum_{i=1}^{M}T^r_i\alpha^r_it^r_i\;, 
    \hat{N}(r) = \sum_{i=1}^{M}T^r_i\alpha^r_i\hat{n}^r_i \;,
\end{equation}
and render the segment label and generalized features along the ray $r$ by 
\begin{equation}
    \label{eq: label and feature}
    \hat{S}(r) = \sum_{i=1}^{M}T^r_i\alpha^r_i\hat{s}^r_i \;,
    \hat{F}(r) = \sum_{i=1}^{M}T^r_i\alpha^r_i\hat{f}^r_i \;,
\end{equation}
where the $\hat{c}^r_i, t^r_i, \hat{n}^r_i, \hat{s}^r_i, \hat{f}^r_i$ represented the color, distance, normal, segment label and feature for points $i$ respectively.

\subsubsection{Front-background Separated Reconstruction}
Unlike the existing decomposed neural implicit surface modeling methods~\cite{wu2022object, kong2023vmap}, which predefined the number of instances and used multiple SDF fields or networks to represent each instance, we distill the generalized features into networks and use it to interactively decompose each object.
Although we can segment most objects by distilled SAM features, 
Specifically, we defined the scene field by $d$ and two signed distance function fields, front ground $d_{front}$ and background $d_{back}$, and their relationship can be derived as $d$ = min($d_{front}$, $d_{back}$).



% Previous version
%
% \subsubsection{Promptable feature field}
% % How to segment things in 3D? 
% Existing methods \cite{siddiqui2022panoptic, kobayashi2022decomposing, goel2022interactive, tschernezki2022neural} have shown that borrowing capabilities from 2D image-based networks has significant potential for this image-based task.
% % Given the objectness from 2D, how to bring it to 3D?
% Objectness is one of the key abilities for accurate decomposition of the holistic scene.
% A significant amount of research \cite{kirillov2023segment, caron2021emerging, li2022language} explores extracting objectness in 2D images, and make notable progress in this area.
% In order to transfer the objectness awareness capabilities from 2D features to 3D neural representation, we follow previous work \cite{kobayashi2022decomposing,goel2022interactive,siddiqui2022panoptic,tschernezki2022neural} and supervise a feature field with a pretrained pixel-level image encoder as a teacher network.
% Motivated by the reasons discussed in the previous sections, we extend the feature field to a promptable feature field based on SAM feature.
% Promptable feature field includes two core design: a distilled feature rendering network and a 3D-2D downsampling mapper.
% For the distilled feature rendering network, given a 3D coordinate $x$, the feature rendering network can be defined as $f_{\theta}$ parameterized by $\theta$ for predicting a rendering feature value by
% \begin{equation}
%   \boldsymbol{\hat{f}} = f_\theta(\boldsymbol{x}).
%   \label{eq:feature rendering network}
% \end{equation}
% Due to the view-independent nature of objectness, we do not need to include the view direction as an additional input to the feature rendering function.
% % Need additional formula ...
% % ----------------------------------------------------------
% % How to obtain pixel_level feature from point_level feature
% % ----------------------------------------------------------
% We can optimize $f_{\theta}$ through minimizing the difference between rendered features $\hat{F}(m, p)$ and teacher's encoder features $F_t(m, p)$ for the same image $m$.
% The feature loss can be represented by
% \begin{equation}
%   \mathcal{L}_{feature} = \sum_{p \in R} ||\hat{F}(m, p) - F_t(m, p)||_1 \text{,}
%   \label{eq:feature loss}
% \end{equation}
% where $R$ represents sampled rays.
% Based on this, the MonoSDF \cite{yu2022monosdf} representation is optimized to minimize the total loss
% \begin{equation}
%   \mathcal{L} = \mathcal{L}_{rgb} + \lambda_{1} \mathcal{L}_{eikonal} + \lambda_{2} \mathcal{L}_{depth} + \lambda_{3} \mathcal{L}_{normal} + \lambda_{4} \mathcal{L}_{feature}
%   \label{eq:field total loss}
% \end{equation}
% for the final field. Due to existence of multi-view inconsistency for teacher feature, we apply stop-gradient strategy to avoid misleading the learning of reconstructed geometry.
% Based on the rendered features, the most straightforward approach is to directly obtain preview dynamic masks by applying a mask decoder from SAM to the image-level features.
% Due to the fixed and small size of the feature map that the mask decoder can accept, we need to downsample the rendering feature map which has the same size with image before passing it to the decoder.
% However, there are two significant drawbacks observed using this approach. 
% Firstly, the obtained masks have severe edge aliasing issues, resulting in jagged edges. 
% Secondly, the quality of the obtained masks is generally low, as demonstrated in the xxx provided.
% The main reasons for these issues are as follows:
% 1.) Explicit downsampling is not suitable for features, leading to information loss.
% 2.) Multi-view inconsistency in the teacher features is optimized during the reconstruction process, resulting in a mismatch between the distilled features and the mask decoder, as shown in Figure xxx.
% To address these issues, we further design a lightweight 3D-2D downsampling mapper to downsample the 3D feature map from the corresponding view to the specified size while aligning them with the feature space of the mask decoder.
% With the proposed mapper, we can obtain accurate and low-aliasing dynamic masks corresponding to any desired viewpoint for preview based on the rendering features.
% With the input of rendered feature map $\hat{F}(m)$ of image $m$, the mapper can be defined as a mapping function $d_{\phi}$ parameterized by $\phi$ for obtaining downsampled feature map by
% \begin{equation}
%   \hat{F}_d(m) = d_{\phi}(\hat{F}(m)).
%   \label{eq:downsampling mapper}
% \end{equation}
% The mapper is a convolutional neural network (CNN) composed of multiple convolution layers and can be trained independently. We thus minimize the mapping loss, $\mathcal{L}_{mapping}$:
% \begin{equation}
%   \mathcal{L}_{mapping} = ||\hat{F}(m) - F_t(m)||_1 \text{.}
%   \label{eq:mapping loss}
% \end{equation}
% The key to solving the problem lies in the fact that this simple and lightweight module discards redundant information effectively and accurately. 
% The downsampling mapper, with its learnable convolutional layers, can adaptively reduce the resolution of the 3D-aware features, ensuring that important information is preserved while discarding unnecessary details.
% Based on the promptable feature field, we obtain 3D-aware promptable features that exhibit both explicit 3D objectness and the ability to generate dynamic masks at the image level from arbitrary view.

% Based on the results obtained from the previous subsections, we propose a novel surface growing algorithm that forms the final piece of the design for promptable automatic decomposition with obtaining meshes with a single interaction. 
% Our objective is to utilize the acquired single-view mask and leverage the learned 3D objectness to extend its perception into the 3D space, ultimately generating a comprehensive 3D mask that accurately delineates the selected object.\\
% Previous works \cite{jambon2023nerfshop, goel2022interactive} employ region growing algorithm to refine the mask in 3D space. 
% However, based on the design of using the region growing algorithm, their method heavily relies on user interaction.
% Considering the accuracy of seed points and the efficiency of growth, we choose the high-confidence boundary of the selected preview as the seed points for region growing.
% The high-confidence boundary is obtained through applying erosion and contour extraction to the selected preview mask.\\
% Based on high-confidence boundary pixels, we obtain the seed points $\mathcal{P}_{seed}$ through depth mapping to project the region to 3D space.
% Additionally, we obtain a growth termination boundary through applying dilation and contour extraction to the selected preview mask.
% Similarly, termination points can be obtained through depth mapping.
% Started with a predefined highest boundary of similarity between points, i.e., $\varphi$, we calculate the similarity between each seed point and all of its neighbours in the same face.
% If the similarity is higher than $\varphi$, we add the corresponding neighbour to the selected point set.
% After the growing based on $\varphi$ checking, all the selected points with at least one unselected neighbour will be updated as seed points.
% Then we update $\varphi$ as $\varphi - step size$ to continuously grow until the number of seed points can be zero, or the number of selected termination points reaches a tolerance threshold, i.e., $\epsilon$.
% The purpose of setting this threshold is to enhance the robustness of the algorithm.\\
% Accordingly, if the selected object view is not suitable, for example, if the selected object occupies only a small number of pixels, the user needs to adjust $\epsilon$ to obtain better results.
% Since we select neighboring points based on faces, we can directly extract a sub-mesh describing the selected object from the rendered mesh based on the selected points.


% \begin{figure}[!t]
%     % \centering
%     \begin{algorithm}[H]
%     \caption{Surface Growing}
%     \begin{algorithmic}
%         \Procedure{SurfaceGrowingAlgorithm}{$P$, $B$, $R$, $C$, $\theta$, $\epsilon$}
%             \State initialization of $DP$, $DP[i][j]$ represents point $P[i]$ is the optimal solution under the threshold $j$
%             \State initialize target vertices $T \gets empty$
%             \State initialize $C' \gets C$ 
%             \For{$i$ from 1 to $|P|$}
%                 \For{$j$ from 1 to $C$}
%                     \State find all of the neighbor points of $P[i]$, $A$ with defined relationship $R$
%                     \For{$a$ in $A$}
%                         \State calculate $similarity \gets \text{CosineSimilarity}(F(a), F(P[i]))$
%                         \If{$similarity > C'$}
%                             \State update $DP[i][j]$ and add $a$ to optimal solutions
%                         \EndIf
%                     \EndFor
%                 \EndFor
%             \EndFor
%             \State find the optimal solutions in $DP[i][j]$ and add corresponding points to $T$
%             \While{ratio $\epsilon$ and $C' \geq \theta$}
%                 \State  $C' \gets C' - \theta$
%                 \State empty $DP$
                
%                 \For{$i$ from 1 to $|T|$}
%                     \For{$j$ from 1 to $C'$}
%                         \State find all of the neighbor points of $T[i]$, $A$ with defined relationship $R$
%                         \For{$a$ in $A$}
%                             \State calculate $similarity \gets \text{CosineSimilarity}(F(a), F(T[i]))$
%                             \If{$similarity > C'$}
%                                 \State update $DP[i][j]$ and ad $a$ to optimal solutions
%                             \EndIf
%                         \EndFor
%                     \EndFor
%                 \EndFor
%                 \State find the optimal solution in $DP[i][j]$ and add corresponding points to $T$
%             \EndWhile
%             \State return $T$
%         \EndProcedure
%     \end{algorithmic}
%     \end{algorithm}
%     \label{fig:enter-label}
% \end{figure}

% \begin{figure}[!t]
%     \centering
%     \begin{algorithm}[H]
%     \caption{Surface Growing}
%     \label{surface_growing_alg}
%     \begin{algorithmic}[1]
%     \Procedure{SurfaceGrowingAlgorithm}{$\mathbb P$, $\mathbb S$, $\mathbb B$, $\Re$, $\mathcal F$, $\tau$, $\theta$, $\epsilon$}
%         \State Initialize the target set $\mathbb T \gets \mathbb S$
%         \State $\mathbb T' \gets \mathbb T$
%         \State initialize the intermediate set $\mathbb I \gets \emptyset$
%         \While{$\mathbb S \neq \emptyset$}
%             \State $\tau' \gets \tau - \theta$
%             \For{$s$ in $\mathbb S$}
%                 \State $\mathbb A \gets \Re(s)$
%                 \For{$a$ in $\mathbb A$}
%                     \State  $similarity \gets \frac{{\mathcal F(a) \cdot \mathcal F(s)}}{{\left\lVert \mathcal F(a) \right\rVert \left\lVert \mathcal F(s) \right\rVert}}$
%                     \If{$similarity > \tau'$}
%                         \State add $a$ to $\mathbb T$
%                         \State add $\Re(a)$ to $\mathbb A$
%                     \Else
%                         \State add $a$ to $\mathbb I$
%                     \EndIf
%                 \EndFor
%             \EndFor
%             \If{ $\frac{\lvert \mathbb T \cap \mathbb B \rvert}{\lvert \mathbb B \rvert} > \epsilon$}
%                 \State return $\mathbb T'$
%             \Else
%                 \State $\mathbb T' \gets \mathbb T$, $\mathbb S \gets \mathbb I$, $\mathbb I \gets \emptyset$
%             \EndIf
%             \State $\tau \gets \tau'$
%         \EndWhile
%     \EndProcedure
%     \end{algorithmic}
%     \end{algorithm}
%     \label{fig:enter-label}
% \end{figure}


==> sec_bak/4_experiments.tex <==
\section{Experiments}
\label{sec:exp}


\subsection{Experiments Setup}
\paragraph{Implimentation Details.} 
Our method is implemented in Pytorch and apply the Adam optimizer with a learning rate of $5e-4$ for the tiny MLP part.
For the geometry MLP, semantic MLP and Feature MLP, we only use two linear layers with 256 nodes.
As for Semantic MLP, we use single MLP with 128 nodes.

In the reconstruction strategy, we minimize the loss
\begin{equation}
\begin{aligned}
    \mathcal{L} = &\mathcal{L}_{rgb} +\mathcal{L}_{geo} +  \lambda_1\mathcal{L}_{O} + \lambda_2\mathcal{L}_{reg} + \\
    &\lambda_3\mathcal{L}_{man} +  \lambda_4\mathcal{L}_{floor} + \lambda_5\mathcal{L}_{sem} + \lambda_6\mathcal{L}_f,\;
\end{aligned}
\end{equation}
to optimize our implicit neural surface, where we set $ \lambda_1, \lambda_2, \lambda_3, \lambda_4, \lambda_5, \lambda_6 $ as $0.1, 0.1, 0.01, 0.01, 0.5, 0.1$, respectively.
More details can be found in the supplementary.

\paragraph{Dataset and Metrics}
Our experiments are mainly conducted on the \textbf{Replica}~\cite{replica19arxiv} dataset, which is a synthetic dataset with each providing meshes, HDR textures and instance annotations.
We follow the selection of ObjSDF++~\cite{wu2023objectsdf++} to evaluate the effectiveness of our method.
We report both instance-level and holistic reconstruction results on this dataset.
To further demonstrate the robustness of our method, we also use the \textbf{ScanNet}~\cite{dai2017scannet} as the real world dataset which provides 1513 scenes.
We select 4 scenes for evaluation and report the number of selection and holistic reconstruction results on it.
The reconstruction results are mainly evaluated by Chamfer-$L_1$ and F-Score. 
More details can be seen in the supplementary.

\paragraph{Compared Methods.}
The compared are mainly divided into two categories. 
The first one is the object compositional reconstruction methods that uses multi fields to represent each objects with the supervision from ground truth instance masks, like ObjSDF++~\cite{wu2023objectsdf++} and vMap~\cite{kong2023vmap}. 
We compare the instance level and holistic scene reconstruction quality with them. 
The second category is the volume density based methods that decompose each scenes with generalized features, like ISRF~\cite{goel2022interactive}, DFF~\cite{kobayashi2022decomposing}.
Since this type of method does not introduce geometric constraints, we mainly compare the way of decomposition.

\subsection{Results}
\paragraph{Object and holistic scene reconstruction on Replica}
To evaluate the decomposed reconstruction capabilities of Total-Decom, we first conduct experiments 
% \begin{table*}[t]
%   \centering
%     \begin{adjustbox}{width=\textwidth}
%   % \scriptsize
%     \small
%   \begin{tabular}{l|ccc||cc|cc}
%     \toprule
%       & \multicolumn{3}{c||}{Model Components} & \multicolumn{2}{c|}{Scene Reconstruction} & \multicolumn{2}{c}{Object Reconstruction} \\
%     % \cmidrule(r){2-4} 
%         Method  & Object Guidance & Mono Cue& Regularizer & Chamfer-L1$\downarrow$ & F-score $\uparrow$ & Chamfer-L1$\downarrow$ & F-score $\uparrow$\\
%     \midrule
%      ObjSDF~\cite{wu2022object} & Semantic &   & & 22.8$\pm$14.8 & 25.74 $\pm$5.70& 7.05$\pm$0.40 & 59.91$\pm$6.67  \\
%      \midrule
%      ObjSDF* & Semantic & \checkmark& & 4.14$\pm$1.53 &78.34$\pm$15.34& 4.65$\pm$0.11& 74.06$\pm$3.12\\
%      % ObjSDF* & Semantic & \checkmark&\checkmark & 3.96 & 80.58 & & \\
%      % Ours w/o &  &  & \\
%      Ours w/o reg& Occlusion Opacity & \checkmark& & 3.60$\pm$ 1.13 & 85.59$\pm$ 8.12& 3.78$\pm$ 0.09& 79.51$\pm$ 2.92\\
%      Ours & Occlusion Opacity & \checkmark&\checkmark & 3.58$\pm$1.08 & 85.69 $\pm$6.55& 3.74$\pm$ 0.09& 80.10 $\pm$ 2.63 \\ 
%     \bottomrule
%   \end{tabular}
%     \end{adjustbox}
%   \caption{\textbf{The quantitative average results from 8 Replica scenes evaluated on scene and object reconstruction}. We compare our results with vanilla ObjectSDF~\cite{wu2022object} and its improved version, ObjSDF* (adding monocular geometry cue).} %(add the multi-resolution grid position encoding on vanilla ObjectSDF).}
%   \label{tbl:com_replica}
%   \vspace{-6mm}
% \end{table*}
\begin{table}[t]
    \centering \scalebox{0.75}{
    \renewcommand\arraystretch{1.3}
    \begin{tabular}{c|cc|cc}
        \bottomrule[0.9pt] & \multicolumn{2}{c|}{Scene Reconstruction} & \multicolumn{2}{c}{Decomposed object Reconstruction} \\
        \textbf{Method} & Accuracy $\downarrow$ & Completeness $\downarrow$ & Chamfer-$\mathcal{L}_1$ $\downarrow$  & F-score $\uparrow$ \\ 
        \hline
        ObjSDF++ & 2.93 & \textbf{4.76} & 3.84 & 79.49 \\
        \hline
        \emph{Ours} & \textbf{2.10} & 5.06 & \textbf{3.58} & \textbf{81.70} \\
        % \textbf{Method} & Chamfer-$\mathcal{L}_1$ $\downarrow$  & F-score $\uparrow$ \\ 
        % \hline
        % ObjSDF++ & 3.80 & 78.23 \\
        % \hline
        % \emph{Ours} & \textbf{3.58} & \textbf{81.52} \\
        \toprule[0.9pt]
    \end{tabular}
        }
    \vspace{-0.3cm}
    \caption{}
    \label{tab:com_2d}
\vspace{-0.1cm}
\end{table}
% \begin{table}[h]
%   \centering
%   % \footnotesize
%   \vspace{3pt}
%   %\tablestyle{6pt}{1}
%   \resizebox{\linewidth}{!}{
%       \footnotesize
%     \begin{tabular}{l|ccc}
%     \hline
%     Method & Normal C.$\uparrow$  &Chamfer-$\mathcal{L}_1$ $\downarrow$  &F-score $\uparrow$ \\
%     \hline
%     Conv-Occ~\cite{peng2020convolutional} & 85.73 & 6.43 & 58.33 \\
%     LIG~\cite{Local_Implicit_Grid_CVPR20} & 89.56& 5.53 & 65.20 \\
%     \hline
%     NICER-SLAM~\cite{zhu2023nicerslam} &90.27 & 3.91 & - \\
%     UNISURF$^\dagger$~\cite{oechsle2021unisurf}         &90.96 &4.93 &78.99 \\
%     MonoSDF$^\dagger$~\cite{yu2022monosdf}         &92.11 &2.94 &86.18 \\
%     \textbf{Ours}$^\dagger$  &\textbf{93.43} &\textbf{2.58} &\textbf{92.12}\\
%     \hline
%   \end{tabular}}
%   \vspace{3pt}
%   \caption{Quantitative assessments of the proposed model against prior works on the Replica dataset. Herein, $^\dagger$ indicates the use of geometry priors as supervision signals.}
%   \label{tab:all in replica}
%   \vspace{-8pt}
% \end{table}
\paragraph{Comparison of interactive methods}
\paragraph{Background reconstruction}
In Fig~\ref{fig: manhattan}, we have already shown the effect of our newly proposed constraint to the background field on the \textit{room\_2} in the Replica dataset.
To demonstrate effectiveness of our method, we also show additional reconstructed results on the more Replica scenes and ScanNet scenes. 

\paragraph{Object and holistic scene reconstruction on in-the wild data}
\paragraph{Scene editing}
\paragraph{Room re-decoration with generative model}
% \subsection{Geometry-driven animating}

==> sec_bak/bk_related_work.tex <==
\section{Related Work}
\label{sec:related_work}
% \vspace{0.1in}
\noindent\textbf{Object Compositional Reconstruction}
In order to better reconstruct the geometry of objects in complex scenes, many research efforts have been devoted to exploring better object-level compositional scene representations. For instance, ObjSDF \cite{wu2022object} proposes a compositional scene representation to assist in geometry optimization in highly composite scenes and object-level extraction with the help of multi-view consistent instance labels. Kong {\etal} \cite{kong2023vmap} build an object-level scene model from a real-time RGB-D input stream for object-compositional SLAM. Wu {\etal} enhance ObjSDF with an occlusion-aware object opacity rendering scheme and further mitigate object occlusions in complex scenes through an object distinction regularization term. 
%Additionally, a new occlusion-aware object opacity rendering scheme is introduced to reduce the negative impact of occlusion on scene reconstruction. 
However, these methods rely heavily on accurate consistent ground-truth instance-level labels and cannot effectively preserve all objects within the reconstruction.
\begin{figure}[t]
% \vspace{-10pt}
    \centering
    \includegraphics[width=\linewidth]{./figure/PCA.pdf}
    \vspace{-15pt}
    \caption{Visualization for distilled generalized features.}
    \label{fig: feature study}
    \vspace{-15pt}
\end{figure}

% \vspace{0.1in}
\noindent\textbf{Decompositional Neural Rendering} Neural radiance fields (NeRFs) offer a unified representation to represent the appearance~\cite{mildenhall2021nerf, yu2021pixelnerf}, and other spatially varying properties~\cite{Kundu_2022_CVPR}. 
In the field of decompositional neural rendering, many research efforts investigate the distillation of generalized features~\cite{lerf2023, goel2022interactive, kobayashi2022decomposing,tschernezki2022neural}, or segmentation predictions~\cite{siddiqui2022panoptic, bing2022dm} from large-scale pre-trained image backbones~\cite{caron2021emerging, oquab2023dinov2,radford2021learning,cheng2022masked}to neural fields. 
% such as DINO~\cite{caron2021emerging, oquab2023dinov2}, CLIP features~\cite{radford2021learning} and panoptic segmentation~\cite{cheng2022masked}, 
Specifically, Semantic NeRF \cite{zhi2021place} explores incorporating regressing semantic labels into the process of Novel View Synthesis.
Building upon this, distilled feature fields (DFFs) \cite{kobayashi2022decomposing} and neural feature fusion fields (N3F) \cite{tschernezki2022neural} have emerged as pioneering approaches for distilling \cite{hinton2015distilling} semantic features~\cite{li2022language, goel2022interactive} from pretrained models into NeRF for decomposition. 
ISRF \cite{goel2022interactive} does not rely solely on feature matching, but instead obtains the results through region growing.
These approaches leverage feature similarities or predicted instance/semantic codes for grouping and implicitly decomposing a scene, offering greater scalability for large-scale scenes.  
However, when directly applied to the reconstruction task, these strategies often produce decomposed outputs that are incomplete and exhibit poorly defined contours (see Fig.~\ref{fig: selected_mesh}) due to ill-defined object boundaries~\cite{goel2022interactive} or inconsistent and low-quality segmentation predictions~\cite{wang2022dm, cheng2022masked, he2017mask} used during training. 
In contrast to existing methods, our work not only avoids the need for extensive manual interaction through a geometry-guided feature approach but enables the extraction of any constituent part of a complex scene.

%\vspace{0.1in}
% \vspace{0.1in}
\noindent \textbf{NeRF with SAM} Recently, segmentation methods based on different representations~\cite{} have developed rapidly. 
SAM~\cite{kirillov2023segment} achieves efficient 2D interactive segmentation capabilities through extensive high-quality annotated supervision. 
It brings forth more possibilities in this field and has the potential to help achieve thorough decomposition of complex scenes with plausible 2D segmentation capabilities. Recently, some concurrent works have explored the combination of SAM and NeRF for decomposition.
SA3D~\cite{cen2023segment} incorporates cross-view self-prompting technique to obtain multi-view consistent masks. However, running SAM multiple times incurs high computational costs, and the segmentation results are sensitive to interaction trajectories, leading to unstable performance.



